Learning to Maximize Mutual Information for Chain-of-Thought Distillation

Knowledge distillation, the technique of transferring knowledge from large, complex models to smaller ones, marks a pivotal step towards efficient AI deployment. Distilling Step-by-Step~(DSS), a novel method utilizing chain-of-thought~(CoT) distillation, has demonstrated promise by imbuing smaller models with the superior reasoning capabilities of their larger counterparts. In DSS, the distilled model acquires the ability to generate rationales and predict labels concurrently through a multi-task learning framework. However, DSS overlooks the intrinsic relationship between the two training tasks, leading to ineffective integration of CoT knowledge with the task of label prediction. To this end, we investigate the mutual relationship of the two tasks from Information Bottleneck perspective and formulate it as maximizing the mutual information of the representation features of the two tasks. We propose a variational approach to solve this optimization problem using a learning-based method. Our experimental results across four datasets demonstrate that our method outperforms the state-of-the-art DSS. Our findings offer insightful guidance for future research on language model distillation as well as applications involving CoT. Codes are available at \url{https://github.com/xinchen9/cot_distillation_ACL2024}.

==> icml2024/content/ack.tex <==
\section*{Acknowledgements}
\label{sec:ack}

 We thank reviewers for providing helpful feedback. 


==> icml2024/content/chainofthoughts.tex <==
\subsubsection{Quality of CoT Examples by GPT-4 Evaluation }
We evaluate the quality of CoT examples using GPT-4, as it achieves the state-of-the-art human alignment performance and is used for text generation evaluation in previous work~\cite{liu2023gpteval,hsu2023gpt,wang-etal-2023-towards}. Inspired by~\cite{wang-etal-2023-towards}, we ask GPT-4 to evaluate the quality of the provided CoT examples based on their coherency and relevancy to the input questions and answers. We randomly sample 50 CoT examples from the four datasets and ask GPT-4 to score based on a scale from 1 to 5, where 1 indicates completely incoherent and irrelevant responses, and 5 represents highly coherent, relevant, and helpful responses. For each sample, we run the same sample for four times to obtain self-consistency to measure the reliability of the responses. Table~\ref{tab:gpt_eval} presents the prompt we use for GPT-4 evaluation,  average scores and standard deviation on the scores obtained over the four datasets. We report the scores on both provided CoT (``gold'') rationales and distilled model predicted rationales. 

\begin{table}[!ht]
\small
\centering
\begin{tabular}{c c c c c}
\toprule
\multicolumn{5}{c}{\textbf{Prompt for GPT 4 Evaluation}} \\ \midrule  
\multicolumn{5}{l}{Given an input pair of a question and an answer of a}\\
\multicolumn{5}{l}{$task name$  task, how good is the given Chain-of-thought} \\
\multicolumn{5}{l}{example? From 1-5, where 1 is completely incoherent and }\\
\multicolumn{5}{l}{irrelevant, 2 is somewhat incoherent and irrelevant, 3 is } \\
\multicolumn{5}{l}{coherent, relevant but not helpful, 4 is somewhat helpful, } \\ 
\multicolumn{5}{l}{and 5 is helpful and it explains the answer well.} \\ 
\midrule
\multicolumn{5}{c}{\textbf{Average Scores and Standard Deviation}} \\ \midrule 
 \textbf{Model}& \textbf{SVAMP} & \textbf{CQA} & \textbf{e-SNLI} & \textbf{ANLI} \\ \midrule 
  Gold &   4.63\scriptsize{$\pm$1.05}  &    3.95\scriptsize{$\pm$1.16}   &   2.42\scriptsize{$\pm$1.23}   &  3.82\scriptsize{$\pm$1.26}  \\ 
  \multicolumn{1}{r}{\scriptsize{\textit{++}}} & 4.43\scriptsize{$\pm$1.18} & 4.11\scriptsize{$\pm$1.40} & 3.49\scriptsize{$\pm$1.35} & 4.01\scriptsize{$\pm$1.10} \\ 
    %\multicolumn{4}{c}{\textbf{Average Scores and Standard Deviation from Our Model}} \\ \midrule 
%  \textbf{SVAMP} & \textbf{CQA} & \textbf{e-SNLI} & \textbf{ANLI} \\ \midrule 
DSS & 2.50\scriptsize{$\pm$1.42}  &    3.60\scriptsize{$\pm$1.61}     &    3.24\scriptsize{$\pm$1.27}   &   3.48\scriptsize{$\pm$1.40}  \\ 
\multicolumn{1}{r}{\scriptsize{\textit{++}}} & 2.53\scriptsize{$\pm$1.46}  &    3.64\scriptsize{$\pm$1.62}     &    3.18\scriptsize{$\pm$1.21}   &   3.44\scriptsize{$\pm$1.30}  \\ 

   Ours & 2.30\scriptsize{$\pm$1.54}  &    3.70\scriptsize{$\pm$1.45}     &    3.03\scriptsize{$\pm$1.47}   &   3.42\scriptsize{$\pm$1.37}  \\ 
   \multicolumn{1}{r}{\scriptsize{\textit{++}}} &  2.72\scriptsize{$\pm$1.45} & 3.63\scriptsize{$\pm$1.60} & 3.17\scriptsize{$\pm$1.17} & 3.34\scriptsize{$\pm$1.21}  \\ 
\bottomrule
\end{tabular}
\caption{Prompt used and results of 50 randomly sampled CoT examples from the four datasets evaluated by GPT-4. We use \textit{++} to denote the setting with \textit{self-consistency} evaluation. }
\label{tab:gpt_eval}
\end{table}

\begin{table}[ht]
\small 
    \centering
    \begin{tabular}{c|c|c|c|c} \toprule
      \textbf{Model} &  \textbf{SVAMP} & \textbf{CQA} & \textbf{e-SNLI} & \textbf{ANLI}  \\  \midrule
      DSS & 0.12 & \textcolor{teal}{0.66} & 0.05  & 0.26 \\ 
      & \scriptsize{$p>0.05$} & \scriptsize{$p<0.05$} & \scriptsize{$p>0.05$} & \scriptsize{$p>0.05$} \\ 
       Ours  &  \textcolor{teal}{0.42}  & \textcolor{teal}{0.53} &  0.03 & 0.26 \\
       & \scriptsize{$p<0.05$} & \scriptsize{$p<0.05$} & \scriptsize{$p>0.05$} & \scriptsize{$p>0.05$} \\  
       \bottomrule
    \end{tabular}
    \caption{ Pearson correlation between CoT quality and accuracy of label prediction on the 50 random samples on the test set. We highlight the correlation with statistical significance ($p<0.05$). }
    \label{tab:my_label}
\end{table}

The effectiveness of our MI-based distillation method is closely linked to the quality of CoT reasoning in the training data. When the CoT quality is high, as in SVAMP, a strong correlation is observed between the model's label prediction accuracy and the quality of its generated CoT. However, this correlation weakens significantly when the CoT quality is low (e-SNLI), suggesting that the model struggles to align label prediction with coherent rationale generation under poor training conditions. Interestingly, with average-quality CoT data (ANLI), the performance gap between our MI-based distillation and DSS is minimal, suggesting that the effectiveness of our approach is particularly reliant on the presence of high-quality reasoning in the training data.



\subsubsection{Case Studies on the Output Rationale}


\begin{figure}[!t]
    \centering
    \includegraphics[width=.5\textwidth]{icml2024/figure/svamp_example.pdf}
    \vspace{-10pt}
    \caption{A case study of the output rationale on SVAMP dataset.}
    \label{fig:svamp_example}
\end{figure}


\begin{figure}[!t]
    \centering
    \includegraphics[width=.5\textwidth]{icml2024/figure/esnli_example.pdf}
    \vspace{-10pt}
    \caption{A case study of the output rationale on e-SNLI dataset. %\hanxian{need to double check the outputs}
    }
    \label{fig:esnli_example}
\end{figure}


We performed case studies on SVAMP and e-SNLI as illustrated in Figure~\ref{fig:svamp_example} and~\ref{fig:esnli_example}. In the SVAMP example, the question asks the difference in the number of kids Julia played with from Monday to Tuesday, with specific numbers provided for Monday, Tuesday, and Wednesday. 
DSS generates an incorrect explanation, which contradicts the given question, resulting in to a wrong answer. 
Conversely, our method correctly identifies the
comparison needed between the number of kids Julia played with on Monday and Tuesday, leading to the correct answer. 
Notably, our generated CoT reasoning is identical to the golden one, demonstrating that by precisely grasping the rationale, our approach effectively resolves the math problem. 
We also show the evaluation results (score and reasoning) from GPT-4, where our method gains a top score of 5 and DSS gains only a mere score of 1. 
This example showcases that the high-quality CoT generated by our method enhances problem-solving capabilities in math tasks like SVAMP.

Another example (Figure~\ref{fig:esnli_example}) is from e-SNLI, where the task is to identify whether the hypothesis is entailment, contradiction, or neutral, based on the given premise and hypothesis. Although both our method and DSS generate the correct label output, it is worth noting that, the CoT of our method points out the relationship between the premise and the hypothesis, while DSS only restates the hypothesis without providing any extra explanation or connecting the hypothesis to the premise. Our generated rationale also gains a higher score than DSS. A higher-quality rationale tends to facilitate more accurate label prediction, thereby enhancing overall task performance.

==> icml2024/content/conclusion.tex <==
\section{Conclusion}
\label{sec:con}
In this paper, we re-investigate the DSS framework from an information-theoretic perspective. We model it using Information Bottleneck and propose to strengthen it by maximizing the mutual information between rationale generation and label prediction tasks. The proposed learning-based method can automatically optimize the CoT distillation and bolster the reasoning ability of the distilled smaller models. Both our qualitative and quantitative analysis demonstrate the rationale behind our method and shed light on aspects of language model distillation and CoT applications.

\section{Limitation}
\label{sec:lim}
Our comparative analysis primarily focuses on the Distilling Step-by-Step (DSS) framework, which serves as our main benchmark. This concentrated comparison, while valuable for a deep understanding of DSS's nuances and our advancements over it, constitutes a limitation of our work. Specifically, our analysis does not extend to a broader range of knowledge distillation methods currently employed in the field, focusing exclusively on T5 and not including other LLMs like Mistral and Llama2, Llama3 model family. This focus may overlook the potential insights and contrasts that could emerge from evaluating our approach against a wider array of distillation techniques. Future research could benefit from a more expansive comparative study, incorporating diverse methodologies to fully contextualize our findings within the broader landscape of knowledge distillation practices. This broader comparison would not only validate the efficacy of our method in various settings but also illuminate areas for further refinement and innovation. 

However, it is important to note that our contribution lies in providing an in-depth analysis from both theoretical and practical viewpoints to enhance the CoT distillation process. Our work delves into the intricacies of utilizing mutual information to improve distillation outcomes, offering significant advancements in understanding and applying CoT distillation techniques. 

\section{Ethical Issues}
\label{sec:ethical}


In this paper, we carefully considered the ethical implications in line with the ACL code of ethics. We evaluated the potential dual-use concerns, ensuring our research serves to benefit society and does not cause inadvertent harm. Our methodology and applications were thoroughly assessed for fairness, non-discrimination, and privacy, particularly in the context of data handling and model outputs. We also ensured our study did not expose any negative impact on individuals and groups. Moreover, we did not engage in academic dishonesty and adhered to high-quality processes and product standards in our professional work. We include this detailed discussion of these ethical considerations, affirming our commitment to responsible and beneficial computational linguistics research.



==> icml2024/content/confidence.tex <==
\begin{table*}[ht]
\centering
\small 
\begin{tabular}{c|cc|cc|cc|cc|cc|cc}
\toprule 
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{SVAMP}} & \multicolumn{2}{c|}{\textbf{CQA}} & \multicolumn{2}{c|}{\textbf{e-SNLI}} & \multicolumn{2}{c|}{\textbf{ANLI}} & \multicolumn{2}{c|}{\textbf{e-SNLI} (Out)} & \multicolumn{2}{c}{\textbf{ANLI} (Out)} \\ 
                       & ECE        & Conf.       & ECE       & Conf.      & ECE         & Conf.        & ECE        & Conf.       & ECE                   & Conf.                  & ECE                   & Conf.                 \\ \midrule 
DSS  & 11.81 & 32.56 & 11.75 & 42.79 & 8.54 & 34.33 & 11.12 & 42.72 & 9.81 & 38.01 & 12.78 & 41.69\\
Ours  & 18.92 & 36.81 & 13.65 & 41.17 & 4.35 & 30.06 & 6.94 & 35.90 & 6.61 & 38.08 & 12.27 & 42.35\\
\bottomrule 
\end{tabular}
\caption{Comparisons of our model and DSS on the expected calibration errors (ECE) and average confidence scores (Conf.). }
\label{tab:calib}
\end{table*}
Calibration measures the alignment between a model's predicted accuracy and its confidence levels. \citeauthor{lee2022hard} (\citeyear{lee2022hard}) introduced an innovative perspective on model distillation, positioning the teacher model not only as a source of knowledge but also as a tool for identifying mis-calibration during the training of the student model. This ability to maintain calibration and make reliable predictions is crucial for downstream applications and has been the focus of prior studies~\cite{chen-etal-2023-close, lee2022hard, jiang2021can}. Here, we apply the Expected Calibration Errors (ECE) and Average Confidence Scores to reflect the alignment between the model's predicted probabilities and the actual outcomes, thereby gauging the reliability and certainty of its predictions. Despite the potential limitations inherent in these metrics, we still employ ECE in our experiments due to its simplicity and popularity, as in previous work on investigating the calibration quality of T5~\cite{chen-etal-2023-close, lee2022hard}.  

We employ a 10-bin-based ECE metric and a softmax-based approach to compute average confidence scores from the test outputs across all four datasets. Given that e-SNLI and ANLI essentially represent the same task, we conduct an out-of-domain experiment by testing the model checkpoint trained on one dataset with the test set of the other. This analysis gives us insights into how well our model generalizes across similar tasks and the robustness of its predictions in out-of-domain scenarios and to assess the calibration quality of the model more comprehensively.  

Table~\ref{tab:calib} presents the results of the distilled model calibration evaluation. Overall, both models report lower ECE and confidence scores on SVAMP and e-SNLI, indicating that these two tasks are more challenging and models are less certain about their prediction. Lower ECE values from our MI-based distillation approach are presented for e-SNLI and ANLI, and their respective out-of-domain tests. Notably, our method achieves an ECE of 4.35 in e-SNLI, significantly lower than DSS's 8.54. However, in SVAMP and CQA, our method records higher ECE, indicating potential areas for improvement in these domains. The trade-off in calibration accuracy in specific tasks like SVAMP and CQA compared to DSS suggests future directions for refining our approach. 

Regarding average confidence scores (Conf.), our method generally maintains competitive confidence levels, with notable improvements in e-SNLI and ANLI. In e-SNLI, the confidence is lower (30.06) compared to DSS (34.33), which, combined with a lower ECE, suggests a more realistic confidence estimation. Conversely, in the out-of-domain scenarios for e-SNLI and ANLI, our method shows marginally higher confidence scores than DSS, which, coupled with the lower ECE, indicates robustness in out-of-domain generalization. 

 %Since we have developed a smaller model distilled from a larger one, we are particularly interested in understanding how well this model can maintain prediction quality, specifically in terms of calibration, that is, how well the model's predicted accuracy aligns with its confidence levels. 
%This performance aspect is critical because the distilled model must replicate the accuracy of its larger predecessor while ensuring its confidence scores accurately reflect prediction likelihoods, a vital characteristic for the model's trustworthiness and usability in decision-making applications where correct interpretation of these scores is essential. We apply the expected calibration errors (ECE) and average confidence scores to reflect the   \cite{chen-etal-2023-close} 
 

==> icml2024/content/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\subsection{Analysis on T5 Calibration} 

\input{icml2024/content/confidence} 

\subsection{Analysis on CoT Output}

\input{icml2024/content/chainofthoughts}

==> icml2024/content/experiment.tex <==
\section{Experiments}
\label{sec:exper}
\subsection{Experimental  Setting}
\paragraph{Datasets.} We conducted the experiments on four widely-used benchmark datasets across three different NLP tasks: e-SNLI~\cite{camburu2018snli} and ANLI~\cite{nie2019adversarial} for natural language inference; CQA~\cite{talmor2018commonsenseqa} for commonsense question answering; and SVAMP~\cite{patel2021nlp} for arithmetic math word problems. We used rationale generated by PaLM 540B~\cite{chowdhery2023palm}, which were collected and open-sourced by~\cite{hsieh2023distilling}\footnote{\label{myfootnote}Data and DSS code are from \url{https://github.com/google-research/distilling-step-by-step}.}.

\paragraph{Setup.} Based on CoT properties and the comparative experimental study in~\cite{hsieh2023distilling}, our work adopted T5-base~(220 million) and T5-small~(60 million) to the student models. 
$\alpha_{1}$ and $\alpha_{2}$ were set as $0.5$ and $\alpha_{3}$ is set as $0.1$. We trained our models on one A100 GPU with $80G$ memory. For T5 base model, the training time for the full-size four dataset was approximately 14.4 hours. For T5 small model, the training times was approximately 8.6 hours.

\paragraph{Baselines.} We compare our work with the state-of-the-art DSS~\cite{hsieh2023distilling} by running their open-sourced code and include two other baseline reported in their work: (1) Standard Finetune, which involves using the prevailing pretrain-then-finetune paradigm to finetune a model with ground-truth labels through standard label supervision.~\cite{howard2018universal}. (2) Single-task, which finetunes the model using both of the label and non-CoT rationale as supervision .  


\paragraph{Evaluation Settings.} Following the DSS work~\cite{hsieh2023distilling}, we adopt the accuracy as the performance metrics across all four datasets. Higher accuracy indicates better results. Besides accuracy, we also adopt Expected Calibration Errors~(ECE) and Average Confidence Scores to evaluate calibration of the T5-base model. A lower ECE and higher Average Confidence Scores indicate better performance. We adopt GPT-4 to evaluate Quality of CoT examples and subjective analysis. Please refer to our codes for more details.


\subsection{Results}

\noindent\textbf{Experiments of T5-base Model.} We present our experimental results for the T5-base model in Table~\ref{tab:basemodel}. In single-task training, the rationale and label are concatenated into a single sequence, which is treated as the target in training models~\cite{hsieh2023distilling}. Our proposed method consistently achieves better performance than standard fine-tuning and single-task methods across all datasets. Compared to DSS, our method outperforms DSS on ANLI, CQA, and SVAMP, and achieves nearly the same accuracy on e-SNLI. 
%$+1.12\%, +7.62\%, +1.69\%, +5.37\%$ accuracy improvement on e-SNLI, ANLI, CQA and SVAMP.

\noindent\textbf{Experiments of T5-small Model.} The experimental results for the T5-small model are shown in Table~\ref{tab:smallmodel}. The patterns of the results are similar to those of T5-base. Our proposed method consistently achieves better performance than standard finetuning across all dataset. Compared to DSS, our method outperforms DSS on ANLI, CQA and SVAMP, and is just 0.2\% less accuracy on e-SNLI.

\noindent\textbf{Distillation with LLM Labels.} We conducted an experiment on e-SNLI and ANLI datasets with T5-base model to evaluate the effect of label quality. We distilled the student models using labels generated by 540B PaLM instead of the ground truth. The results are shown in Table~\ref{tab:my_label_llm}. Comparing Table~\ref{tab:basemodel} and Table~\ref{tab:my_label_llm}, we observe the label quality affects the distillation results in both methods. Even With the noisy LLM labels, our model still outperforms DSS on both datasets.

\noindent\textbf{Distillation with smaller datasets.} To evaluate the performance of our models on smaller datasets, we distilled T5-base and T5-small models on various sizes of four datasets and compared to DSS method. The results are shown in Figure.~\ref{fig:smalldataset_t5_base} and ~\ref{fig:smalldataset_t5_small} respectively. 



\begin{table}[!t]
\small
    \centering
    \begin{tabular}{c|c|c|c|c}
    \toprule
        & e-SNLI & ANLI & CQA & SVAMP\\
       \midrule
       Standard FT  & 88.38  & 43.58 & 62.19 &62.63 \\
         \midrule
        Single-task & 88.88 & 43.50 &61.37  & 63.00\\
         \midrule
         DSS & \textbf{89.51} & 49.58 & 63.29 & 65.50\\
         \midrule
         Ours& 89.50 & \textbf{51.20} & \textbf{63.88} & \textbf{68.00}\\
         \bottomrule
    \end{tabular}
    \caption{CoT distillation results on T5-base model. The results of Standard Fine-tune (FT), single-task and DSS methods are from~\cite{hsieh2023distilling}. %Our proposed method leads to better performance than other methods on three datasets. Only on e-SNLI dataset, our method is almost same as DSS. %The results of Finetuning, single-task and DSS methods are from~\cite{hsieh2023distilling}. %Finetuning is standard finetuning method, input is text and output is label.  
    }
    \label{tab:basemodel}
\end{table}
\label{sec:accuracy}

%\subsection{Results with small dataset}


\begin{table}[!tb]
\small
    \centering
    \begin{tabular}{c|c|c|c|c}
    \toprule
        & e-SNLI & ANLI & CQA & SVAMP\\
        \midrule
         Standard FT &  82.90 & 42.00 & 43.16 & 45.00\\
         \midrule
         DSS & \textbf{83.43} & 42.90 & 43.24 & 48.00\\
         \midrule
          Ours & 83.23 & \textbf{43.70} & \textbf{43.90} & \textbf{52.50}\\
         \bottomrule
    \end{tabular}
    \caption{CoT distillation results on T5-small model. %Our proposed method leads to better performance then other methods on three datasets. Only on e-SNLI dataset, our method is slight less than the DSS. %We ran three methods with same training configuration of~\cite{hsieh2023distilling} 
    }
    \label{tab:smallmodel}
\end{table}

\begin{table}[!tb]
\small
    \centering
    \begin{tabular}{c|c|c} \toprule
      \textbf{Model} &  e-SNLI & ANLI  \\  \midrule
      DSS & 82.65  & 42.80 \\  
       Ours  & 82.81  & 45.50 \\
       \bottomrule
    \end{tabular}
    \caption{Results on two dataset on T5-base model with LLM generated labels.%, showing that the quality of labels directly affect performance on both methods.
    }
    \label{tab:my_label_llm}
\end{table}


\subsection{Ablation Study}
\paragraph{Effectiveness of Difference Dimension Reduction Method}
In our proposed MI loss module, we utilize maximum reduction to align the dimensions of different features. Additionally, mean reduction serves as an alternative method for dimension reduction, based on the hypothesis that important features can represent better than average features. In Table~\ref{tab:mean_max}, we present the results of two different layer of MI module. The results indicate the superiority of the MI module with maximum reduction.
% So far, we have focused on exhibited the effectiveness of our proposed method. In this section, we perform further studies to understand inference of different components and loss functions in MI module loss. Specifically, we study 1) MI module design, max reduction VS mean reduction and 2): auxiliary loss design, cross entropy vs KD loss. 
\paragraph{Comparison with KL Divergence} KL divergence loss has been extensively utilized in KD tasks,serving as a metric for assessing the similarity between two data distributions ~\cite{Hinton2015distilling,zhang2022contrastive,gou2021knowledge,husain2024distributionally}. While KL divergence is widely applied in various KD scenarios, modeling DSS using IB framework has proven to be more accurate than using similarity measures, as discussed in Section~\ref{sec:meth}. To validate our hypothesis, we conducted experiments on T5-base model across all four datasets. As shown in Table~\ref{tab:KL_CE}, our proposed method consistently outperforms the KL divergence approach, demonstrating superior performance.  
% and has been widely used in a variety of KD tasks. However, model DSS using IB is more accurate than using similarity, as discussed in Section~\ref{sec:meth}. In order to verify our theory, we conduct an experiment on T5-base model with all four dataset. As  shown in Table~\ref{tab:KL_CE}, Our proposed method consistently achieves better performance compared with KL divergence. 
% For DSS, the two tasks are insufficient and unnecessary. As a result, KD is not well-suitable for our work. In Table~\ref{tab:KL_CE}, we report the results that use KD loss as the auxiliary loss. The results have shown that our proposed method outperforms the method using KD loss as the auxiliary loss.   
\begin{table}[!t]
\small 
    \centering
    \begin{tabular}{c|c|c|c|c}
    \toprule 
        & e-SNLI & ANLI & CQA & SVAMP\\
        \midrule 
         Mean &  89.34 & \textbf{51.40} & 63.88 & 66.50\\
         \midrule 
         Max& \textbf{89.50} & 51.20 & \textbf{63.88} & \textbf{68.00}\\
         \bottomrule
    \end{tabular}
    \caption{Results of Mean Reduction Vs Maximum Reduction on T5-based model.  }
    \label{tab:mean_max}
\end{table}

\begin{table}[!ht]
\small 
    \centering
    \begin{tabular}{c|c|c|c|c}
    \toprule
        & e-SNLI & ANLI & CQA & SVAMP\\
        \midrule
         KL Divergence &  89.42 & 42.00 & 62.49 & 67.00\\
         \midrule
         Ours& \textbf{89.50} & \textbf{51.2} & \textbf{63.88} & \textbf{68.00}\\
         \bottomrule 
    \end{tabular}
    \caption{Results of KD loss  VS our proposed cross entropy loss, on T5-base model. }
    \label{tab:KL_CE}
\end{table}


% \begin{figure*}[!ht]
% \begin{multicols}{2}
%     \includegraphics[width=\linewidth]{icml2024/figure/anli.png}\par 
%     \includegraphics[width=\linewidth]{icml2024/figure/cqa.png}\par 
%     \end{multicols}
% \begin{multicols}{2}
%     \includegraphics[width=\linewidth]{icml2024/figure/esnli.png}\par
%     \includegraphics[width=\linewidth]{icml2024/figure/svamp.png}\par
% \end{multicols}
% \caption{caption here}
% \end{figure*}

\begin{figure*}[!t]
\vskip 0.2in
\begin{center}
% \centerline{\includegraphics[clip,trim= {.15\columnwidth} 0 {.15\columnwidth} 0, width=0.9\columnwidth]{icml2024/figure/scheme.png}}
\centerline{\includegraphics[width=2\columnwidth]{icml2024/figure/smalldata.pdf}}
\caption{Comparison with DSS with varying sizes of training datasets on T5-base model.}
\label{fig:smalldataset_t5_base}
\end{center}
\vskip -0.2in
\end{figure*}

\begin{figure*}[!t]
\vskip 0.2in
\begin{center}
% \centerline{\includegraphics[clip,trim= {.15\columnwidth} 0 {.15\columnwidth} 0, width=0.9\columnwidth]{icml2024/figure/scheme.png}}
\centerline{\includegraphics[width=2\columnwidth]{icml2024/figure/small_model_diff_size.pdf}}
\caption{Comparison with DSS with varying sizes of training datasets on T5-small model.}
\label{fig:smalldataset_t5_small}
\end{center}
\vskip -0.2in
\end{figure*}




==> icml2024/content/intro.tex <==
\section{Introduction}
\label{sec:intro}
% Recently, Chain-of-Thought (CoT) prompting methods have shown language models models~(LMs) have exhibited enhanced reasoning capabilities in tackling complex reasoning tasks, owing to the utilization of a method named
% “Chain-of-Thought (CoT) prompting”.

%The capabilities of larger language models~(LLMs) grow with regarding to their size leading to considerable demand for resources~\cite{chowdhery2023palm}. Consequently, deploying these models in real world application is challenging, and the development of of efficient LLMs has become one of hot topics~\cite{wan2023efficient,yang2023harnessing,ding2023efficiency}.  

\begin{figure*}[!ht]
\vskip 0.2in
\begin{center}
% \centerline{\includegraphics[clip,trim= {.15\columnwidth} 0 {.15\columnwidth} 0, width=0.9\columnwidth]{icml2024/figure/scheme.png}}
\centerline{\includegraphics[width=1.8\columnwidth]{icml2024/figure/MI_overview.pdf}}
\caption{Overview on our approach: distilling step by step from an IB perspective and measuring intrinsic relationship between the two tasks by MI. The DSS is a MTL framework pipeline consisting of 
%two tasks: 
predicting and explaining tasks. 
%In the predicting task, the input is \textsc{[predict]+text} and output is label, and in the explaining task, the input is \textsc{[explain]+text} and output is rationale generated by CoT. 
Besides prediction loss and explanation losses used in DSS, we design an auxiliary loss,named MI loss, which aims to maximize the mutual information between the two representation features. In turns, CoT reasoning capacity can be enhanced by task-oriented distillation.}
\label{fig:scheme}
\end{center}
\vskip -0.2in
\end{figure*}

The capabilities of larger language models (LLMs) tend to scale with their model size, leading to a substantial demand for memory and compute resources~\cite{chowdhery2023palm,wei2022emergent}. Distilling knowledge from large LLMs to smaller LLMs has been pivotal for efficient AI deployment~\cite{Hinton2015distilling,phuong2019towards,wei2022chain}. Chain-of-Thought~(CoT) model distillation represents a pivotal advance in the quest to imbue smaller language models with the sophisticated reasoning capabilities of their larger counterparts. By distilling complex thought processes into more compact models, this approach aims to democratize access to advanced natural language understanding and reasoning across a wider array of computational resources.    %This poses challenges in the practical deployment of LLMs for real-world applications. 
%To circumvent these deployment challenges, recent research efforts~\cite{wan2023efficient,yang2023harnessing, ding2023efficiency} have pivoted towards efficient LLMs.
%the development of efficient LLMs has emerged as a critical area of focus in recent research, as highlighted by works such as \cite{wan2023efficient,yang2023harnessing, ding2023efficiency}.
%One main stream is knowledge distillation (KD), which transfers knowledge from larger, more competent teacher models into smaller student models affordable for practical applications~\cite{Hinton2015distilling,phuong2019towards}.
%Chain-of-thought (CoT), which prompts to breaks down complex tasks into smaller, more manageable steps, enhances LLM's problem solving ability 
%prompting has been proposed to improve LLMs' ability, 
%especially on the challenging arithmetic, commonsense, and symbolic reasoning tasks~\cite{wei2022chain}.
%, represents a significant advancement in enhancing the cognitive abilities of LLMs. 
%This approach involves a prompting mechanism that breaks down complex tasks into smaller, more manageable steps, thereby enhancing the effectiveness of the problem-solving process. 
However, it has been observed the CoT prompting methods on a model with less than 10 billion parameters may not only fail to enhance model performance but also potentially impair it~\cite{wei2022chain}. 
This challenge has spurred the exploration of training smaller language models that possess enhanced reasoning capabilities through CoT%, marking an exciting development in the field of efficient LLMs training
~\cite{ma2023sci,magister2023teaching,li2023symbolic}.

%Since its emerging~\cite{Hinton2015distilling}, Knowledge Distillation (KD) has been widely applied to a wide range of applications~\cite{phuong2019towards}.
%KD has become a powerful tool to transfer knowledge either in various ML tasks such as efficient AI for training smaller models~\cite{jiao2020tinybert}, MTL for enhancing main task training~\cite{yang2022cross}, and omin-supervision learning with data distillation~\cite{radosavovic2018data}.le
%Leveraging KD and CoT, a 
A recent research effort \textit{Distilling Step-by-Step}~(DSS)~\cite{hsieh2023distilling} proposes to efficiently train smaller student models %with shared weights 
guided by the rationales generated by a significantly larger teacher model, leveraging both CoT and KD. Instead of training both teacher and student models, it prompts the large teacher model to generate CoT rationales, and applies multi-task learning (MTL) framework to train a smaller models for both label and rationale prediction.  %generated from the teacher model are collected through employing CoT prompting. 
%In the online distillation stage, it applies multi-task learning~(MLT) to train a smaller student model to predict both labels and rationales.%, as shown in Figure~\ref{fig:scheme}. %Intuitively, rationales provide richer, more detailed information about why an input is mapped to a specific output label, allowing the small student model to forecast labels more accurately.
%Building on CoT reasoning, Hsieh et al.~\cite{hsieh2023distilling} have recently developed a novel two-step training pipeline, namely \textit{Distilling Step-by-Step}~(DSS). 
%This pipeline is designed to train smaller LMs more effectively or on less data. 
%In the first step of this process, a larger model, acting as a teacher, employs CoT prompting to generate both answers and rationales. 
%The second step involves applying multi-task learning~(MLT), aiming to minimize both label loss and rationale loss. 
%Essentially, DSS is an MLT task that enables the transfer of reasoning capabilities from LLMs to smaller LMs during the rationale prediction task. 
In this process, CoT knowledge is transferred through rationales generated by LLMs to smaller models via MTL.  
The smaller model enhances its reasoning capabilities by learning to predict rationales, which in turn improves its ability to predict labels accurately.
%as it demands fewer resources during training and leads to smaller models with enhanced reasoning ability. 
Different from conventional knowledge distillation~\cite{Hinton2015distilling}, larger teacher models perform inference only once to generate rationales, without any model updating in distillation. Only smaller student models are trained and optimized, leading to a smaller distillation cost. DSS thus offers significant benefits in terms of both efficiency and effectiveness.
%Obviously, this greatly reduces the demands for resources. 
% Through the transfer of CoT reasoning, smaller models can reach performance levels on reasoning tasks that were previously unattainable due to their inherent limitations. 
% This approach is particularly useful in scenarios with limited computational resources or where deploying large models is impractical due to processing or storage constraints.~\cite{brown2020language,zhao2023survey}. %Besides efficiency, the DSS framework enables a significant enhancement to the smaller models by imbuing them with the sophisticated reasoning capabilities typically associated with LLMs. 
% %It is worth noting that larger teacher models is only run forward part during the first step to generate rationales, while only the smaller models are run during training step.


% %Figure~\ref{fig:scheme} illustrates the DSS training process, in which the input text is combined with task prefixes \textsc{[predict]} and \textsc{[explain]}. These tokens signify two distinct tasks: label \textit{predicting} task and CoT rationale \textit{explaining} task, from the same input text. \hanxian{duplicated with the figure caption}
% While DSS aims to promote knowledge distillation for complex tasks, low-quality and noisy CoT rationales, and the intricacies in training models under the MTL framework could impact the effectiveness and reliability of the DSS process~\cite{wang-etal-2023-scott}. LLMs are prone to producing hallucinations and inconsistent rationales, which could potentially mislead the student model toward incorrect answers and cause conflicts in MTL that destruct student model learning~\cite{wang-etal-2023-scott,mueller2022text}.  

%Compared with general knowledge distillation, DSS adopts MTL framework to transfer the knowledge through the shared weights instead of two models. Consequently, we can consider the DSS as one type of self-distillation. However, previous self-distillation works train one larger model and improve some shallow sub-networks with task-orient the knowledge~\cite{zhang2019your, xu2019data,zhang2020task}. 

Research works of both MTL and KD have shown that introducing auxiliary losses improves performance of either main task of MTL or student models of distillation. However, DSS fails to bridge the predicting and explaining tasks. DSS aims to promote knowledge distillation for complex tasks, low-quality and noisy CoT rationales, and the intricacies in training models under the MTL framework could impact the effectiveness and reliability of the DSS process~\cite{wang-etal-2023-scott}. Furthermore, LLMs are prone to producing hallucinations and inconsistent rationales, which %could 
potentially mislead the student model toward incorrect answers and cause conflicts in MTL that destruct student model learning~\cite{mueller2022text}.

%To this end, 
To tackle the issues, we investigate the DSS from an information-theoretic viewpoint and develop a new auxiliary loss that aims to maximize the mutual information of the two tasks. %shared between the auxiliary task CoT rationale generation and the main task within an MTL framework. 
Our focus %is on 
lies in how the label-predicting task can generate representations that maximally align with those produced by the explaining task, thereby enhancing %the 
knowledge transfer from CoT. We conceptualize this relationship as task-oriented self-distillation, specifically designed to maximize mutual information (MI). MI plays a pivotal role in the quality of representations learned by these tasks. Despite the challenges in directly estimating MI, we draw inspiration from the methodology outlined in~\cite{covert2023learning} and propose a novel variational method to effectively maximize MI in the DSS context. 

We conduct comprehensive experiments with two smaller types of T5 models~\cite{2020t5}, T5-base~(220M) and T5-small~(60M), on four popular datasets. These datasets are e-SNLI~\cite{NIPS2018_8163}, ANLI~\cite{nie2019adversarial}, CQA~\cite{talmor-etal-2019-commonsenseqa} and SVAMP~\cite{patel-etal-2021-nlp}. Meanwhile, we provide deep and detailed analysis on Section~\ref{sec:discussion}. We believe that these results will be a guide for using DSS framework in the future.  

% The emergence of large language models (LLMs) has significantly revolutionized the NLP landscape, as highlighted by \citeauthor{brown2020language} and \citeauthor{zhao2023survey}. One of the key trends in this field is leveraging the capabilities of LLMs to unlock new applications, particularly in transferring the reasoning capacity of these models to smaller ones. This transfer is facilitated by the Distilling Step-by-Step (DSS) process, which utilizes a Multi-Task Learning (MTL) pipeline.  

%\citeauthor{wei2022chain} introduced Chain-of-thought as a powerful technique that enhances AI models' cognitive abilities by breaking down complex tasks into smaller steps. They point out that these prompting methods that are less than 10 billion parameters not only fail to enhance performance but can potentially impair it. As a result, training smaller LLM models that have reasoning capabilities via COT has evolved into intriguing research fields within the realm of efficient LLMs~\cite{ma2023sci,magister2023teaching,zhu2023survey,ding2023efficiency}. Compared with others, the most prominent benefits of DSS are efficient and effective, meaning less demand for resource during training and achieving smaller models with better accuracy.

%Introduced in~\cite{wei2022chain}, Chain-of-thought reasoning is

%Recently, Hsieh~\etal~\cite{hsieh2023distilling} has developed a simple two-step training pipeline, \textit{referring to as Distilling step-by-step~(DSS)}, to training smaller language models models~(LMs) on less data. The first step is data generation step, in which considering a larger model, as a teacher, Chain-of-Thought~(CoT) prompting is utilized to generate both answers and rationales. The second step is training step, in which multi-task learning~(MLT) is applied to minimize both label loss and rationale loss. DSS is de facto MLT task but can transfer the reasoning capabilities of LLMs into smaller model during training rationales predict task.


%Introduced in~\cite{wei2022chain}, Chain-of-thought reasoning is a powerful technique that enhances AI models' cognitive abilities by breaking down complex tasks into smaller steps. At the same time, Wei~\etal point out that these prompting methods that are less than 10 billion parameters not only fail to enhance performance but can potentially impair it. As a result, training smaller LLM models which have reasoning capabilities via COT has evolved into intriguing research fields within the realm of efficient LLMs~\cite{ma2023sci,magister2023teaching,zhu2023survey,ding2023efficiency}. Compared with others, the most prominent benefits of DSS are efficient and effective, meaning less demand for resource during training and achieving smaller models with better accuracy.
% Recent work have found that these CoT prompting methods are effective only for models with at least 10 billion of parameters~\cite{wei2022chain,Liu2023FederatedPA}. Leveraging MLT, the goal of DSS is to transfer 

%Since emergence of the LLMs the NLP landscape has been revolutionized~\cite{brown2020language,zhao2023survey}. Utilizing their new capacities to unlock new applications is a trend. Through MTL pipeline, DSS transfers reasoning capacity of COT generated by LLMs to small models.    

%Although success transferring capacities of COT of larger models, two things sounds be overlooked: noise label and how impacts of MLT because of the special relationship of the two tasks. As shown in Fig.~\ref{fig:scheme}, the training of SDD can be decomposed into two tasks, one refers to as predicting task, in in which the input is [PREDICT] + text and output is label and one refers to as explaining task, which the input is [EXPLAIN]+ text and the output is rationale. In the inference phase, only predicting task is evaluated. It is obvious that the explaining task is an auxiliary task in DSS. 
 
% Both MLT and noise label training are well-studied problems, and we also believe that some methods of MLT and noise label. However, this paper aims to analyze DSS which is a new scenario because of emerging of LLMs and focus on deeply understanding the method with perceptive of information theory. In term of it, we propose a new loss to improve the training pipeline.

% In terms of \cite{covert2023learning}, 





%Exploiting useful information contained in training tasks and formulating them into training paradigm are important in MTL. On the other hand, COT and the main task are not sufficient and necessary relationship. In this paper, we investigate properties of two tasks from an information-theoretic perspective. For better transferring knowledge from COT, the predicting task needs to generate representations that share maximum information with the representations generated by explaining task. Based on this intuition, we formulate the relationship between two task as dynamic feature selection through self-learning for maximizing mutual information~(MI), which plays an important role in the quality of the representations they learn.However, it is hard to directly estimate MI. In this paper, Inspired by learning method to maximize MI in~\cite{covert2023learning}, we propose a new variation method to maximize MI method. 
% Mutual information is a fundamental quantity that measures the relationship between random variables but it is notoriously difficult to measure. An exact estimate is only
%tractable for discrete variables or a small set of problems




The main contributions are summarized as below:
\begin{enumerate}
\item  We offer a critical reevaluation of the DSS framework, identifying and addressing its limitations by harnessing an information-theoretic viewpoint that underscores the synergy between label prediction and rationale explanation. 
\item Building on the theoretical foundation, we introduce an innovative auxiliary loss function designed to seamlessly integrate these two tasks. This methodological enhancement not only strengthens the connection between predicting and explaining within the DSS framework but also represents a significant leap forward in our ability to distill complex reasoning into more compact models. %We revisit the DSS training pipeline and formulate the two tasks, predicting and explaining tasks, from an information-theoretic perspective. Based on it, we improve DSS with an auxiliary loss that effectively bridge two tasks. % revisit is not a contribution 
\item  Our methodology demonstrably outperforms existing benchmarks across multiple datasets, evidencing the efficacy of our approach in enhancing the reasoning capabilities of distilled models. % Based on the proposed loss, our method substantially surpasses existing state-of-the-art approaches with significant improvement of most of the cases in four datasets. 
\item We systematically review predicted task and explainable tasks relationships under MTL training task with theoretical analysis results. To the best of our knowledge, it is the first work to quantitative analyze the models with CoT distillation. \hanxian{The last sentence is over-claimed?}
\end{enumerate}

% $$\underset{x \to \infty}{\lim}$$
% $\sum\limits_{j=0}^{3} {2 \above j}$ 

==> icml2024/content/method.tex <==
\section{Methodology}
\label{sec:meth}

%\begin{figure*}[!ht]
%\vskip 0.2in
%\begin{center}
%% \centerline{\includegraphics[clip,trim= {.15\columnwidth} 0 {.15\columnwidth} 0, width=0.9\columnwidth]{icml2024/figure/scheme.png}}
%\centerline{\includegraphics[width=1.85\columnwidth]{icml2024/figure/loss.png}}
%\caption{Overview on training loss desgin. The DSS is a MTL framework pipeline consisting of two tasks: predicting and explaining tasks. In the predicting task, the input is \textsc{[predict]+text} and output is label, and in the explaining task, the input is \textsc{[explain]+text} and output is rationale generated by COT.}
%\label{fig:loss}
%\end{center}
%\vskip -0.2in
%\end{figure*}


% \label{sec:loss}
This section begins with an introduction to preliminaries of IB. Following this, we formulate our CoT distillation idea within the IB framework and propose a learning approach to optimize MI.  
%we describe our problem of feature section problem with information-theoretic perspective and a learning method to maximize MI. Finally, we discuss the train losses.  
 % the mutual information (MI) of two random variables is a measure of the mutual dependence between the two variables. More specifically, it quantifies the "amount of information" (in units such as shannons (bits), nats or hartleys) obtained about one random variable by observing the other random variable. The concept of mutual information is intimately linked to that of entropy of a random variable, a fundamental notion in information theory that quantifies the expected "amount of information" held in a random variable.
% \subsection{Preliminaries}
% \label{sec:prel}

% Bayes' theorem:
%  \begin{equation}
% \label{eq:bayer}
% P(A|B) = \dfrac{P(B|A)P(A)}{P(B)}
% \end{equation}

%  \begin{equation}
% \label{eq:mi_ineqation}
% \max{(H(X), H(Y))}\leq H(X,Y)\leq(H(X) + H(Y))
% \end{equation}

%  The joint entropy measures how much uncertainty there is in the two random variables X and Y
% taken together

%  \begin{equation}
% \label{eq:mi}
% \mathrm{\mathbf{I(x,y)}} = \sqrt{(g_{x}^{p}-g_{x}^{gt})^2 + (g_{y}^{p}-g_{y}^{gt})^2}
% \end{equation}

 
\subsection{Preliminaries}
\label{section:pr}
% The Information Bottleneck~(IB)~\cite{tishby2015deep,slonim2002information} provides an information-theoretic principle for representation learning, which preserves complex intrinsic correlation structures over high dimensional data. %all information relevant for predicting label while minimizing the redundancy. 

% On the basis of IB~\cite{tishby2015deep,zhang2022improving,wang2019deep}, we formulate our CoT distillation problem with MTL as an optimization problem. 
Under the DSS framework, the prefixes \textsc{[predict]} and \textsc{[explain]} will be prepended to the input text, \textsc{text}, for tasks corresponding to label prediction and rationale generation, respectively. In the label prediction task, given the input \textsc{[predict] + text} along with predictive labels $\mathbf{Y}$, a representation feature $\mathbf{V}$, where $\mathbf{V} \in \mathbb{R}^{d}$, is trained using $\mathbf{Y}$. Similarly, in the rationale generation task, the input \textsc{[explain] + text} and rationale label $\mathbf{R}$ guide the training of a representation feature $\mathbf{Z}$, where $\mathbf{Z} \in \mathbb{R}^{d}$, using $\mathbf{R}$.%As a result, t
% The model weight $w$ is shared by the two tasks.

% As shown in Figure~\ref{fig:scheme}, the goal of the CoT distillation module 
% is to preserve $\mathbf{Z}$ maximally informative to $\mathbf{Y}$, which can be measured by MI:

Our goal is to distill CoT knowledge from larger LLMs to smaller LLMs models. To achieve this, based on the basis of IB~\cite{tishby2015deep,zhang2022improving,wang2019deep}, we model the DSS as following:
%Therefore, the training cab  measured by MO     
% Given the representation features $\mathbf{Z}$ and the prediction label
\begin{equation}
\label{eq:def}
    I(Z;Y) = \int p(z,y) \log \frac{p(z,y)}{p(z)p(y)}dzdy.
\end{equation}
where sampling observations $z \thicksim \mathbf{Z}$ and $v \thicksim \mathbf{V}$. Here $p(\cdot)$ represents the probability distribution.

To encourage CoT distillation to focus on the information represented in label $\mathbf{Y}$,  we propose using IB to enforce an upper, bound $I_{c}$,  on the information flow from the representation features $V$ to the representation features $Z$. This is achieved by maximizing the following objective:

\begin{equation}
\label{eq:bound}
    \max I(Z;Y)  \ \  s.t. \ \ I(Z;V) \leq I_{c} .
\end{equation}
% Hence, maximizing MI $I(Z;Y)$ is equivalent to maximizing $I_{c}$. 
By employing Lagrangian objective, IB allows $Z$ to be maximally expressive about $Y$ while being maximally compressive regarding the input data, as follows:
\begin{equation}
\label{eq:la}
    \mathcal{C}_{IB} = I(Z;V) - \beta I(Z;Y)  
\end{equation}
where $\beta$ is the Lagrange multiplier. Clearly, Eq.~\ref{eq:la} demonstrates the trade-off optimization between high mutual information and high compression~\cite{zhang2022improving,alemi2016deep}. In our scenario, given a predefined small student model, the compression ratio is fixed. Therefore, we formulate the CoT distillation as an optimization problem:
\begin{equation}
\label{eq:max}
    \max I(Z;V)
\end{equation}
Due to symmetric property of MI, $I(Z;V) = I(V;Z)$. CoT distillation can also enhance rationale generation task with the label knowledge. This is validated in Section ~\ref{sec:discussion}.   
    
\subsection{Variational Bounds of MI}
% According to work in~\cite{poole2019variational,covert2023learning}, a tractable variational upper bound can be built by introducing a variational approximation $q(z)$ to the intractable marginal $p(z) = \int dx p(x)p(z|x)$. According to symmetry of MI, $I(Z,V) = I(V,Z)$. So we can rewrite the $I(Z;V)$ of Eq:~\ref{eq:bound}:

% \begin{equation} \label{eq:bound}
% \begin{split}
% I(Z;V) & = \mathbb{E}_{p(z)} \Big[ \frac{p(z|v)}{p(z)} \Big] \\
%  & = \mathbb{E}_{p(z,v)} \Big[ \frac{p(z|v)q(z)}{p(z)q(z)} \Big] \\
%  & = \mathbb{E}_{p(z,v)} \Big[ \frac{p(z|v)}{q(z)} \Big] -KL(p(y)\|q(y))

% \end{split}
% \end{equation}
% \begin{equation} 
% \label{eq1}
% \begin{split}
% I(Z;V) & = \mathbb{E}_{p(z,v)}\Big[ \log \frac{p(z|v)}{p(z)} \Big] \\
%   & = \mathbb{E}_{p(z,v)} \Big[ \frac{p(z|v)q(z)}{p(z)q(z)} \Big] \\
%   & = \mathbb{E}_{p(z,v)} \Big[ \frac{p(z|v)}{q(z)} \Big] - KL(p(z)||q(z)) \\
%   & \leq \mathbb{E}_{p(z,v)} \Big[ \frac{p(z|v)}{q(z)} \Big]
% \end{split}
% \end{equation}
We rewrite $I(Z;V)$ of Equation~\ref{eq:max} as follows: 
{%\small
\begin{equation}
    \label{eq:mi}
    I(Z;V)  = \mathbb{E}_{p(z,v)}\Big[ \log \frac{p(v|z)}{p(v)} \Big]
\end{equation}
}
According to ~\cite{poole2019variational,covert2023learning}, a tractable variational upper bound can be established by introducing a variational approximation $q(v)$ to replace the intractable marginal $p(v)$, demonstrated by:

%\small
\begin{equation} 
\label{eq1}
\begin{split}
I(Z;V) & = \mathbb{E}_{p(z,v)} \Big[\log \frac{p(v|z)q(v)}{p(v)q(v)} \Big] \\
  & = \mathbb{E}_{p(z,v)} \Big[ \log \frac{p(v|z)}{q(v)} \Big] \\
  & - KL(p(v)||q(v))
\end{split}
\end{equation}
here $KL[\cdot||\cdot]$ denotes Kullback-Leibler divergence. The bound is tight when $q(v) = p(v)$. Consequently, $KL(p(v)||q(v))$ is equal to $KL(p(v)||p(v))$, which becomes zero. Therefore, we can derive at the following inequality:
% the upper bound defined in Eq.~\ref{eq:bound} as following:
% \begin{align}
% \label{eq:rewr}

%     I_{c} \approx \mathbb{E}_{p(z)} [D_{KL}((p(z|v)||p(z))]
%     %D_{KL}(p(\mathbf{z}; \mathbf{y} | v) || p(\mathbf{x}_{i} | x_{s}) p(\mathbf{y} | x_{s}) ) 
% \end{align}
% {
% \small
% \begin{equation}
%    I(Z;V) \leq \mathbb{E}_{p(z,v)} \Big[ \log \frac{p(z|v)}{q(v)} \Big]
% \end{equation}
% }
{%\small
\begin{equation}
   I(Z;V) \leq \mathbb{E}_{p(z,v)} \Big[ \log \frac{p(z|v)}{p(v)} \Big]
\end{equation}
}

% \begin{equation} 
% \label{eq2}
% \begin{split}
% I(Z;V)) & \approx \max (\mathbb{E}_{p(z,v)} \Big[ \log \frac{p(z|v)}{p(v)}  \Big] )\\
% &= \max \sum p(z,v) \log \frac{p(v|z)}{p(v)} \\
% &= \max(\sum p(z|v)p(v)\log(v|z) )\\
% &- \max (\sum p(z|v)p(v) \log(p(v))
% & = - \max(\sum p(v) p(z|v)\log(v|z) )
% \end{split}
% \end{equation}
We can then express the MI from Eq.~\ref{eq:mi} as the follows:
{
%\small
\begin{equation}
 \label{eq2}  
 \begin{split}
 \mathbb{E}_{p(z,v)} \Big[ \log \frac{p(z|v)}{p(v)}  \Big]
 &= \sum p(z,v) \log \frac{p(v|z)}{p(v)} \\
 &= \sum p(z|v)p(v)\log p(v|z)  \\
 &- \sum p(v) p(z|v)\log p(v)
 \end{split}
\end{equation}
}
Assuming that  $p(v)$ is uniform distribution for maximal entropy~\cite{schroder2020estimating}, the term $\sum p(v) p(z|v)\log p(v)$ is considered as a constant. This also allows for the omission of $p(v)$ in $\sum p(z|v)p(v)\log p(v|z)$. By combining Eq.~\ref{eq:mi} and Eq.~\ref{eq2}, then maximization of $I(Z;V)$ can be expressed as:

%\small
\begin{equation}
 \label{eq3}  
 \begin{split}
 \max I(Z;V) &= \max \mathbb{E}_{p(z,v)} \Big[ \log \frac{p(z|v)}{p(v)}  \Big]\\
 &\varpropto \max  \sum p(z|v) \log p(v|z) \\
 &= \max ( -\sum p(z|v) \log \frac{1}{p(v|z)} )\\
 & =\min ( \sum p(z|v) \log \frac{1}{p(v|z)} ) \\
 &= \min(\sum CE(z|v, v|z))
 \end{split}
\end{equation}
here $CE$ represents cross entropy. Accordingly, CoT distillation in Eq.~\ref{eq:max} is transformed into the problem outlined in the above equation. This problem can be addressed with a learning-based method. To tackle this issue, we have developed a new MI loss that minimizes cross-entropy of representation features of the rationale generation~($p(z|v)$) and representation
features of the label prediction~($p(v|z)$), effectively maximizing MI during CoT distillation process.
%Finally, estimating the maximum of MI equals to minimize cross entropy.   

% \begin{align}
%     KL(q \Vert u) &= \sum q \log \frac{q}{u}\\
%         &={\textstyle \sum q \log q} - \textstyle \sum q { \log u}\\
%         &=- H(q) - \text{constant}\\
%         \max {\textit{KL}}(q \Vert u) &= \max ~(- H(q) - \text{constant}) \\
%         \max {\textit{KL}}(q \Vert u) &= \min H(q)
% \end{align}


% Blahut–Arimoto algorithm~\cite{naiss2012extension,lin2011algorithm} provides an iterative approach to solve an optimization problem. Here, we consider step-by-step predicted by model $f$, and the expected loss is:
% \begin{equation}
%     \mathbb{E}_{z,v}[l(Z,V)\frac{p(z,y)}{p(z)p(y)]
% \end{equation}
% Therefore, we formalize it in the following proposition for self-distillation task
% \begin{proposition}
%     When $\mathbf{V}, \mathbf{Z}$ is discrete, $l$ is cross-entropy loss. Minimizing the loss of representation features $\mathbf{V}, \mathbf{Z}$ equals to $max\, I(Z;Y)$ in Eq.~\ref{eq:bound}.
% \end{proposition}
% In terms of it, the self-learning process is equivalent to minimizing the one-step-ahead loss.

% \input{icml2024/content/new_prelim}
% \subsection{MI Loss Module Design}
% \label{sec:mi}
% In order to effectively learn knowledge directly guided by the prediction task, we develop a simple and effective module, named MI loss module, to distill CoT knowledge, as shown in Figure~\ref{fig:scheme}. This module consists of softmax and max reduction layers. The softmax layer aims to produce the an output distribution over representation learning space, and the max reduction aims to reduce the dimension of representation features of the label prediction task {\small $\mathbb{R}^{m\times d} \rightarrow \mathbb{R}^{1\times d}$ } and the dimension of representation features of the rationale generation task {\small $\mathbb{R}^{n\times d} \rightarrow \mathbb{R}^{1\times d}$ }.  
\subsection{Training Loss}
\label{sec:loss}
The training loss is given by
\begin{equation}
    \mathcal{L}_{total} 
%( \boldsymbol \theta, \boldsymbol \psi; \mathcal D) 
= \alpha_1 \mathcal{L}_{\mathrm{prediction}} + \alpha_2 \mathcal{L}_{\mathrm{generation}} + \alpha_3 \mathcal{L}_{\mathrm{CE}}
\label{eq: dur_los}
\end{equation}
where $\alpha_1$, $\alpha_2$ and $\alpha_3$ are regularization parameters, all of which are non-negative. $\mathcal{L}_{\mathrm{prediction}}$ represents the loss of the label prediction task, and $\mathcal{L}_{\mathrm{generation}}$ represents the loss of the rationale generation task. Both are general cross-entropy loss as defined in~\cite{hsieh2023distilling}.   
% The prediction loss function is be defined as:
% {
% \small
% \begin{equation}
%     \mathcal{L}_{\mathrm{prediction}} = l(\mathbf{Y}, \hat{\mathbf{Y}})
% \end{equation}
% }
% which calculates the main task~(label prediction task), in which the input is [PREDICT]+ text and output is label $Y$. In our work  $l$ is cross entropy loss. 

% The generation loss is defined as
% {
% \small
% \begin{equation}
%     \mathcal{L}_{\mathrm{generation}} = l(\mathbf{R}, \hat{\mathbf{R}}) 
% \end{equation}
% }
% which calculates the generation loss, in which the input is [EXPLAIN]+ text and output is generated rationale, and target $R$ is generated by 540B PaLM model~\cite{chowdhery2023palm}. 
According to the last line of Equation~\ref{eq3}, we define the our MI loss as
\begin{equation}
    \mathcal{L}_{\mathrm{CE}} = l(f(\mathbf{Z}),f(\mathbf{V}))
\end{equation}
$f$ represents our proposed mutual information (MI) loss module, and $l$ denotes the cross-entropy loss. As shown in Figure~\ref{fig:scheme}, the MI loss module consists of softmax and max reduction layers. The softmax function separately calculates the distributions for the outputs of the vocabulary spaces in the label prediction and rationale generation tasks. Subsequently, a max reduction operation is employed to reduce the dimensionality of the predicted outputs from both tasks to a uniform dimension for the loss calculation. Specifically, in the label prediction task, dimensions are reduced from $\mathbb{R}^{m \times d}$ to $\mathbb{R}^{1 \times d}$, and in the rationale generation task, from $\mathbb{R}^{n \times d}$ to $\mathbb{R}^{1 \times d}$.   %The softmax layer aims to generate an output distribution over representation learning space, while the max reduction aims to reduce the dimension of representation features of the label prediction task {\small $\mathbb{R}^{m\times d} \rightarrow \mathbb{R}^{1\times d}$ } and the dimension of representation features of the rationale generation task {\small $\mathbb{R}^{n\times d} \rightarrow \mathbb{R}^{1\times d}$ }.  

%The $V$ is the feature vectors with the predicted task and $Z$ the feature vectors with the explainable  task. As a result, the MI loss offers a capacity to distill CoT knowledge aligning with main task. According to Equation~\ref{eq3}, minimizing the MI loss %{\small $\mathcal{L}_{\mathrm{MI}}$
%} 
% is to maximize MI $I(Z;Y)$.

% \begin{align}
%     \mathcal{L}_{\mathrm{prediction}} = l(\mathbf{Y}, \hat{\mathbf{Y}}) \nonumber \\
%     \mathcal{L}_{\mathrm{explanation}} = l(\mathbf{R}, \hat{\mathbf{R}}) \nonumber \\
%      \mathcal{L}_{\mathrm{MI}} = l(\mathbf{Z},\mathbf{V})
% \end{align}







==> icml2024/content/new_intro.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure*}[!ht]
\vskip 0.2in
\begin{center}
% \centerline{\includegraphics[clip,trim= {.15\columnwidth} 0 {.15\columnwidth} 0, width=0.9\columnwidth]{icml2024/figure/scheme.png}}
\centerline{\includegraphics[width=2\columnwidth]{icml2024/figure/MIOverview_updated.pdf}}
\caption{Overview of our approach: CoT distillation from an IB perspective and measurement of the intrinsic relationship between the two tasks by MI. The DSS is an MTL framework pipeline comprising label prediction and rationale generation tasks. 
%In the predicting task, the input is \textsc{[predict]+text} and output is label, and in the explaining task, the input is \textsc{[explain]+text} and output is rationale generated by CoT. 
\textit{H} represents the entropy of representation features \textit{V} and \textit{Z}. Besides prediction loss and explanation losses used in conventional DSS, we design an auxiliary loss module to maximize MI between the two representation features. This process enhances CoT reasoning capacity through knowledge distillation.}
\label{fig:scheme}
\end{center}
\vskip -0.2in
\end{figure*}

The capabilities of larger language models (LLMs) tend to scale with their model size, leading to a substantial demand for memory and compute resources~\cite{chowdhery2023palm,wei2022emergent}. Distilling knowledge from larger LLMs to smaller LLMs has been crucial for the efficient deployment of AI~\cite{Hinton2015distilling,phuong2019towards}. Chain-of-Thought (CoT)~\cite{wei2022chain} distillation represents a pivotal advance in the quest to endow smaller language models with the sophisticated reasoning capabilities of their larger counterparts. By distilling complex thought processes into more compact models, this approach aims to democratize access to advanced natural language understanding and reasoning across a wider array of computational resources~\cite{ma2023sci,magister2023teaching,li2023symbolic}. %However, it has been observed the CoT prompting methods on a model with less than 10 billion parameters may not only fail to enhance model performance but also potentially impair it~\cite{wei2022chain}. 
%This challenge has spurred the exploration of training smaller language models that possess enhanced reasoning capabilities through CoT
.

\textit{Distilling Step-by-Step} (DSS)~\cite{hsieh2023distilling} introduces a CoT distillation method that guides smaller models using rationales from LLMs within a multi-task learning (MTL) framework, training them for both \textit{label prediction} and \textit{rationale generation} tasks. 
This framework simultaneously optimizes the model for two related objectives on the same input, enhancing its chain-of-thought learning by sharing representations between the two tasks, thereby improving overall performance efficiently. While DSS brings out the benefits of reducing computational costs, it suffers from the same problem as the conventional MTL framework, that is the difficulty in effectively connecting the prediction and generation tasks. %Despite its aim to enhance knowledge distillation for complex tasks and manage low-quality, noisy CoT rationales, 
The intricacies inherent in training models within the MTL framework can undermine the effectiveness and reliability of the DSS process~\cite{wang-etal-2023-scott}. Despite the successful setup of an MTL framework in DSS, where the tasks of label prediction and rationale generation are intrinsically related, the current configuration may not optimally capture and maximize the mutual knowledge between these tasks. Furthermore, LLMs are prone to producing hallucinations and inconsistent rationales, which %could 
potentially mislead the student model toward incorrect answers and cause conflicts in MTL that destruct student model learning~\cite{mueller2022text}.

% This approach enhances students' reasoning and accuracy by leveraging LLM-generated rationales without requiring teacher model updates. The key challenge in MTL is how to combine learning signals from multiple tasks into one model\cite{caruana1997multitask}. The ways to address this challenge rely on establishing a relationship between tasks. However, it is even harder for DSS because of specific relationships and model structure. The two tasks of DSS, referred to as predicting task and explaining task, are heavily dependence but insufficient and unnecessary. Furthermore, the model of DSS is entirely shared by both two tasks and lack task-owned components. This leads to challenge of extracting intermediate features representing different tasks.  




%To this end, 
To address this issue, we  %successfully 
model the DSS using information bottleneck and investigate it from an information-theoretic viewpoint~\cite{tishby2015deep}. %Based on it, we propose a knowledge distillation~(KD) method to preserve task-specific training of DSS. What is more, estimating MI from finite data is known to be a difficult problem~\cite{mcallester2020formal}. %We also design a varitional method to maximize mutual information (MI). MI plays a pivotal role in the quality of representations learned by tasks, but estimating the mutual information from finite data is known to be a difficult problem~\cite{mcallester2020formal}.
Subsequently, we formulate the DSS as an optimization problem to maximize mutual information~(MI) of label prediction and rationale generation tasks. However, estimating MI from finite data has historically been a difficult problem in both deep learning and information theory~\cite{mcallester2020formal,belghazi2018mutual,paninski2003estimation}. 

In this study, we introduce a variational method to estimate the MI. %Recently, knowledge distillation has been used for solving the challenge of preserving task-specific training in MTL~\cite{li2020knowledge}. Consequently, 
We propose a practical yet effective auxiliary loss to quantify the shared information between the prediction and the generation tasks, thereby enhancing the alignment between the two tasks and facilitating the knowledge transfer from CoT.  
% model tasks of the DSS using Information Bottleneck and investigate it from an information-theoretic viewpoint~\cite{tishby2015deep}. Based on it, we propose a knowledge distillation~(KD) method to preserve task-specific training of DSS. What is more, estimating MI from finite data is known to be a difficult problem~\cite{mcallester2020formal}. %We also design a varitional method to maximize mutual information (MI). MI plays a pivotal role in the quality of representations learned by tasks, but estimating the mutual information from finite data is known to be a difficult problem~\cite{mcallester2020formal}.
% Based on it, we formulate the DSS as an optimization problem to maximize mutual information~(MI) of label prediction and rationale generation tasks. However, estimating MI from finite data is known to be a difficult problem~\cite{mcallester2020formal}. In this study, we introduce a variational method to estimate the MI. Given the model structure of DSS, we develop a simple but effective loss module to distill knowledge from predicting task to explaining task, as shown in Fig.~\ref{fig:scheme}.  the  MI loss modules 
% Recently, knowledge distillation has been used for solving the challenge of preserving task-specific training in MLT~\cite{li2020knowledge}. As a consequence, a practical but effective auxiliary loss is proposed to quantize the shared information between the predicting and explaining tasks, thereby enhancing the alignment between two tasks and ultimately the knowledge transfer from CoT.       
%Our focus lies in how the label-predicting task can generate representations that maximally align with those produced by the explaining task, thereby enhancing 
%knowledge transfer from CoT. We .  Despite the challenges in directly estimating MI, we draw inspiration from the methodology outlined in~\cite{covert2023learning} and propose a novel variational method to effectively maximize MI in the DSS context. We design develop a new auxiliary loss that aims to maximize the mutual information (MI) of the two tasks.  
% We conduct comprehensive experiments with two smaller types of T5 models~\cite{2020t5}, T5-base~(220M) and T5-small~(60M), on four popular datasets. These datasets are e-SNLI~\cite{NIPS2018_8163}, ANLI~\cite{nie2019adversarial}, CQA~\cite{talmor-etal-2019-commonsenseqa} and tSVAMP~\cite{patel-etal-2021-nlp}. 
We conduct comprehensive experiments with two smaller types of T5 models~\cite{2020t5}, T5-base~(220M) and T5-small~(60M), on four popular datasets. Furthermore, we provide detailed analysis in Section~\ref{sec:discussion}. %We believe that these results will be a guide for using the DSS framework in the future.  
Our main contributions are summarized below: 
\squishlist
\item  We reframe the MTL framework of DSS as a MI estimation challenge, aiming to maximize the MI between label prediction and rationale generation tasks. To achieve this, we introduce a variational approach grounded in the IB principle for effective MI estimation. 
To the best of our knowledge, we present the first work of improving CoT distillation from an IB perspective. %with both theoretical justification and a practical solution. %We offer a critical reevaluation of the DSS framework, identifying and addressing its limitations by harnessing an information-theoretic viewpoint that underscores the synergy between label prediction and rationale explanation. 
\item Beyond establishing a theoretical foundation, we present a practical approach for MI estimation, incorporating a simple yet effective auxiliary loss to learning to maximize MI and enhance DSS. %Building on the theoretical foundation, we introduce an auxiliary loss function designed to seamlessly integrate these two tasks. This methodological enhancement not only strengthens the connection between predicting and explaining within the DSS framework but also represents a significant leap forward in our ability to distill complex reasoning into more compact models. 
\item  Our methodology demonstrably outperforms existing benchmarks across multiple datasets, evidencing the efficacy of our approach in enhancing the reasoning capabilities of distilled models. 
\item We conduct a systematic review of the relationship between label prediction and rationale generation tasks under MTL training, presenting both qualitative and quantitative analysis results.
%We systematically review predicted and explainable tasks relationship under MTL training with qualitative and quantitative analysis results. %To the best of our knowledge, it is the first work to quantitative analyze the models with CoT distillation. \hanxian{The last sentence is over-claimed?}
\squishend

Armed with theoretical proofs and experimental results, we aim to lay the groundwork for future research on enhancing CoT distillation within an effective MTL framework, guided by principles from information theory.

==> icml2024/content/new_prelim.tex <==


% \subsection{Preliminaries}

In this section, we lay the foundation for our approach to mutual information-based distillation in a multi-task learning framework using the T5 model. We consider two primary tasks: label prediction and rationale generation, both derived from the same input. Our target smaller model, T5 and its variants, could be considered as a function mapping an input sequence of tokens to an output sequence of tokens.

Since mutual information is nonlinear and can effectively represent the dependencies of features, it is one of widely used measurements in feature selection

We denote $X$ as the input to the model. We define two random variables, $Y_1$ and $Y_2$, representing the outcomes of the label prediction and rationale generation tasks, respectively. The model estimates probability distributions for these tasks, $P_{\text{label}}(Y_1|X)$ for label prediction and $P_{\text{rationale}}(Y_2|X)$ for rationale generation. To adapt the input for MTL, we prepend task-specific prefixes \textsc{predict} and \textsc{explain} to $X$, resulting in modified inputs $X'_{\text{label}}$ and $X'_{\text{rationale}}$. Consequently, the probability distributions are denoted as $P_{\text{label}}(Y_1|X'_{\text{label}})$ and $P_{\text{rationale}}(Y_2|X'_{\text{rationale}})$ for label prediction and rationale generation tasks, respectively.


\subsection{Mutual-Information Based Distillation}
Our distillation process aims to train a smaller model to mimic the behavior of the LLM in performing these two tasks. The key metric guiding this process is the cross-entropy between the probability distributions of the label prediction and rationale generation tasks.

It is rare difficult to directly estimate mutual information in high dimension, especially when involving latent variable optimization

We propose the MI-based distillation approach aims to align the model's understanding and representation of the input $X$
X in such a way that it optimally informs both the label prediction and rationale generation tasks. 
The cross-entropy between these distributions is given by:
\begin{equation}
H(P_{\text{label}}, P_{\text{rationale}}) = -\sum_{y_1} P_{\text{label}}(y_1|X) \log P_{\text{rationale}}(y_1|X)
\end{equation}

This measure quantifies the expected number of additional bits required to identify an outcome of $Y_1$ using the probability distribution of $Y_2$, given the input $X$. Minimizing this cross-entropy is equivalent to maximizing the mutual information between the label prediction and rationale generation tasks, which can be conceptually represented as:
\begin{equation}
\max I(Y_1; Y_2) \approx \min H(P_{\text{label}}, P_{\text{rationale}})
\end{equation}

The distillation process involves adjusting the parameters of the smaller model to minimize the cross-entropy between the two probability distributions, thereby maximizing the mutual information between the label prediction and rationale generation tasks. %This approach ensures that the distilled model efficiently captures and leverages the shared information between these tasks. Next, we explain 

\subsection{A Variational Perspective on MI}

 In this section, we provide a variational perspective, specifically focusing on Conditional Mutual Information (CMI), to further refine our understanding of how information is shared and optimized in our multi-task learning framework using the T5 model. The CMI, denoted as $I(\mathbf{x_{i}}; \mathbf{y} | x_{s})$, is a pivotal concept in dynamically selecting features or tokens that are most informative for tasks, in our work, the label prediction and rationale generation tasks.

In this framework, $x_{s}$ represents the subset of features already selected, $\mathbf{x_{i}}$ represents a candidate feature for selection, and $\mathbf{y}$ represents the output variable, which could be either the label prediction ($Y_1$) or the rationale generation ($Y_2$), depending on the task. The CMI is defined as the KL divergence between the joint and factorized distributions of these variables:
\begin{equation}
I(\mathbf{x_{i}}; \mathbf{y} | x_{s}) = D_{KL}(p(\mathbf{x_{i}}, \mathbf{y} | x_{s}) || p(\mathbf{x}_{i} | x_{s}) p(\mathbf{y} | x_{s}) )
\end{equation}

The feature selection policy, $\phi(x_s)$, aims to minimize this CMI, effectively choosing features that maximize the information about the output variable $\mathbf{y}$. This approach aligns with our objective of distilling and transferring knowledge efficiently in the multi-task T5 framework, where the internal representation of input tokens play a crucial role in predicting both labels and generating rationales.

The prediction function $f$, in the context of T5, is defined as:
\begin{equation}
f(x_{s}) = p(\mathbf{y} | x_{s})
\end{equation}
representing the model's probability estimation of the output given the selected features.

Following the methodologies outlined in ~\cite{covert2023learning,poole2019variational}, we estimate the CMI by calculating the mean KL divergence relative to the model's prediction across different subsets of features:
\begin{equation}
\label{eq:mean}
M_{i}^{n} = \frac{1}{n} \sum_{j=1}^n D_{KL}(p(\mathbf{y} | x_{s}, x_{i}^j) || \frac{1}{n} \sum_{l=1}^n p(\mathbf{y} | x_{s}, x_{i}^l) )
\end{equation}
This estimation process allows us to approximate CMI practically and efficiently, facilitating the dynamic selection of features in our model. Ultimately, as proposed by \cite{covert2023learning}, the limit of this CMI estimator as $n \to \infty$ approaches the true CMI:
\begin{equation}
\lim _{n \to \infty} I_{i}^n = I(\mathbf{y}; \mathbf{x}_{i} | x_{s})
\end{equation}

This variational perspective on mutual information is crucial in our multi-task learning setting. It guides the selection method as an optimization problem, aiming to minimize the expected loss of the model's prediction. The expected loss for adding a new feature $\mathbf{x}{i}$ to the current set $x{s}$ is represented as:
\begin{equation}
\label{eq:expection}
\mathbb{E}_{\mathbf{y}, \mathbf{x}_{i} | x_{s}} = [l(f(x_{s} \cup \mathbf{x}_{i}), \mathbf{y})]
\end{equation}
In the context of MLT framework with T5, the expected loss (if defined in terms of cross-entropy) would guide the feature selection process to minimize the average discrepancy in predictions across different tasks. This formulation aligns with our overarching goal of enhancing the T5 model's efficiency in handling multiple tasks by optimally selecting the most informative features for label prediction and rationale generation.

In terms of the Blahut–Arimoto algorithm, we can obtain
\begin{proposition}
    When $\mathbf{y}$ is discrete, $l$ is cross-entropy loss.The $f$ is the explaining model, and Eq.~\ref{eq:expection} is minimized by predicting model or equal to $\arg max_{i}I(\mathbf{y}; \mathbf{x}_{i} | x_{s})$.
\end{proposition}
In terms of it, the self-learning process is equivalent to minimizing the one-step-ahead loss.
    




==> icml2024/content/old_prelim.tex <==
%Let $\mathbf{x} = (\mathbf{x}_{1}, ...,~\mathbf{x}_{d})$ denotes a vector of input features with dimension $d$, and $\mathbf{y}$ a response variable for a supervised learning task. We notate $s \subseteq [d] \equiv \{1,...d\}$ to denote a subset of indices and $\mathbf{x}_{s} = \{ \mathbf{x}_{i}: i \in s \}$ a subset of features. Bold symbols $\mathbf{x},\mathbf{y}$ represent random variables. The symbols $x,y$ are possible values, and  $p(\mathbf{x},\mathbf{y})$ denotes the \textcolor{red}{joint distribution of(?)} data. 

%Our goal is to design a method to control which features are selected or weighted given the  currently available information. The selection method can be viewed as function $\phi(x_s) \in [d]$, meaning that it selects a subset of features as its input. 

Given a network $f$ and s subset of dataset $x_{s}$, the predicted result can be written as 
\begin{equation}
\label{eq:cost}
% \hat{y} = f(\{x_{i_{t}}\}^{k}_{t=1})
\hat{y} = f(x_{s})
\end{equation}

Given a loss function $l(\hat{y}, y)$ that measures prediction $\hat{y}$ and labels $y$. The cost function is defined as a a policy-predictor pair $(\phi,f)$ as follows:
 \begin{equation}
\label{eq:cost}
% \mathbf{\rho_{k}(\phi,f)} = \mathbb{E}_{p(x,y)}[l(f(\{x_{i_{t}}\}^{k}_{t=1}), \mathbf{y})]
\mathbf{C(\phi,f)} = \mathbb{E}_{p(x,y)}[l(f(x_{s}), \mathbf{y})]
\end{equation}
The goal is to minimize cost function, or to maximize our final predictive accuracy. 

\subsection{A Variational Perspective on MI}
\label{sec:Variation}
The CMI, denoted as $I(\mathbf{x_{i}}; \mathbf{y} | x_{s})$, is defined as the KL divergence between the joint and factorized distributions \textcolor{red}{ of what? }:
\begin{equation}
    I(\mathbf{x_{i}}; \mathbf{y} | x_{s}) = D_{KL}(p(\mathbf{x_{i}}; \mathbf{y} | x_{s}) || p(\mathbf{x}_{i} | x_{s}) p(\mathbf{y} | x_{s}) )
\end{equation}
where the policy as $\phi(x_s) \equiv \arg\min_{i} I(\mathbf{x_{i}}; \mathbf{y} | x_{s}) $, so that features are sequentially selected as to maximize the information about the response variables. The function $f$ is considered as with 
\begin{equation}
    f(x_{s}) = p(\mathbf{y} | x_{s})
\end{equation}
According to ~\cite{covert2023learning,poole2019variational}, We calculate the mean prediction and the mean of KL divergence relative to this prediction, which yields to the CMI estimator as following:
\begin{equation}
\label{eq:mean}
    M_{i}^{n} = \frac{1}{n} \sum_{j=1}^n D_{KL}(p(\mathbf{y} | x_{s}, x_{i}^j) || \frac{1}{n} \sum_{l=1}^n p(\mathbf{y} | x_{s}, x_{i}^l) )
\end{equation}
In terms of \cite{covert2023learning}, the solution of limiting result of Equation~\ref{eq:mean}
\begin{equation}
    \lim _{n \to \infty} I_{i}^n = I(\mathbf{y}; \mathbf{x}_{i} | x_{s})
\end{equation}
% % According to IB priciple~\cite{tishby2015deep}, Given data 
% The goal of dynamic feature selection features with minimal budget that achieve
% The CMI, denoted as $I$

For our propose, the selection method can be viewed as an optimization problem, the expected loss of one step is written as:
% \begin{euqation}
%      \mathbb{E}_{\mathbf{y}, \mathbf{x}_{i} | x_{s}}[l(f(x_{s}), \mathbf{y})
% \end{euqation}
\begin{equation}
    \mathbb{E}_{\mathbf{y}, \mathbf{x}_{i} | x_{s}} = [l(f(x_{s} \cup \mathbf{x}_{i}), \mathbf{y})]
\end{equation}


==> icml2024/content/relatedwork.tex <==
\section{Related Work}
\label{sec:related}
% \paragraph{Distilling Step-by-Step VS Knowledge Distillation} Since proposed by Hinton~\etal~\cite{Hinton2015distilling}, knowledge distillation, referring to transferring knowledge from a teacher to a student model, has been considered as one of most effective way to obtain smaller models and improve model accuracy~\cite{gou2021knowledge,wang2021knowledge}. In general, there are two models, teacher and student models, which have same inputs and targets in KD training pipeline~\cite{Hinton2015distilling}. In recent years, self-distillation~\cite{zhang2021self,zhang2022contrastive},
% \paragraph{COT and LLMs}
% How to effectively transfer the knowledge from these powerful LLMs into smaller models has therefore become an area
% of research interest 
% \paragraph{Multi-task Learning} aims to improve generalization of a
% certain task by learning from other tasks~\cite{caruana1997multitask,zhang2021survey}. It has
% been widely studied in machine learning [6, 12]. The growing interests in learning the relationship between tasks gives
% rise to a number of multitask and transfer learning training
% benchmarks and challenges. 

% Most of existing MLT models have their task-oriented 


% Entropy usage as a risk measure

% There is an extensive literature on binarization for degraded document
% images, but here we mention just a few relevant papers on Sauvola’s method.
% Some surveys are found in [4, 14, 18], and recently developed approaches are
% presented in the annual contest of binarization for degraded document images
% from 2009 to 2014 [19, 20, 21, 22, 23].
We present an overview of previous work across three areas related to our study: knowledge distillation, multi-task learning, and information bottleneck. 
%In this paper we revisit DSS from an information perspective starting from IB. DSS is a training pipeline which majorly involves KD and MTL research areas. 
% Therefore, we mention just some relevant papers.      
% a framework involving KD and MTL, through an IB perspective.

%DSS involves a variety of advanced machine learning techniques, such as KD~\cite{Hinton2015distilling,gou2021knowledge,wang2021knowledge}, MLT~\cite{zhang2021survey,crawshaw2020multi}, CoT~\cite{wei2022chain,chu2023survey}.%,  information theory about machine learning training~\cite{miles2022itrd,tishby2015deep,chen2016infogan},  and training with noise labels~\cite{song2022learning,sukhbaatar2014training,reed2014training}. 
%There is extensive literature on them, but here we mention just some relevant papers on knowledge distillation and information bottleneck with mutual information estimation,  which we make contributions to.  


\noindent\textbf{Knowledge Distillation~(KD)} Originally designed to train small models by leveraging the extensive knowledge of larger models~\cite{Hinton2015distilling}, KD has since been extended to a variety of applications, owwwing to its effective transfer of knowledge across models and tasks~\cite{chen2021distilling,wang2021knowledge,sanh2019distilbert,jiao2020tinybert,luo2024diff,go2023aligning,zhang2022wavelet}.
%The crucial questions are what knowledge to transfer and how to transfer. 
A crucial yet open challenge is how to effectively transfer the knowledge. 
To address the issue, previous studies~\cite{zhang2022contrastive,allen-zhu2023towards,zhang2021self} have extracted various features and designed auxiliary loss functions to enhance KD. 
%designing various some modules to extract different features and auxiliary loss functions has proven to be a successful approach~\cite{zhang2022contrastive,allen-zhu2023towards,zhang2021self}. 
Our work %emphasizes knowledge distillation specifically on 
focuses on improving the model by acquiring mutual knowledge to address both label prediction and rationale generation tasks.
%by addressing the aspects of the mutual knowledge learned by the model in solving label prediction and rationale generation tasks. 
% In general, knowledge distillation works on two or more models, teacher and student models. 
% In recent years, self-distillation techniques have emerged, in which some auxiliary shallow outputs of some sub-networks are optimized by the large model output as well~\cite{allen-zhu2023towards,zhang2021self,zhang2020task}. 
% In our work, the self-distillation aims to a whole and shared weight model.    

\noindent\textbf{Multi-Task Learning~(MTL)} By exploiting commonalities and differences among relevant tasks, MTL can enhance learning efficiency and improve prediction accuracy by learning multiple objectives from a shared representation~\cite{caruana1997multitask,zhang2021survey}. In recent years, MLT has been broadly applied to NLP tasks~\cite{worsham2020multi,zhang2023survey,liu-etal-2019-multi}. However, some studies have identified that training multiple tasks trained simultaneously could lead to conflicts among them, making it challenging to optimize the performance of all tasks simultaneously~\cite{kendall2018multi,lin2019pareto}. 
Recently, KD has also been applied within MTL frameworks, achieving state-of-the-art results in various applications~\cite{li2020knowledge,xu2023multi,yang2022cross,garner2023knowledge,zhang2023blind}. 
%Compared with related works, there are two challenges of DSS in MTL with distillation: 1): Since the predicting and explaining are insufficient and unnecessary  but heavily dependence, it is hard to model it; and 2): The goal of the DSS paradigm is to improve the predicting task instead of both tasks.     
% The underlying idea of MTL is to extract and leverage the knowledge and information shared across the tasks to improve the overall performance or main task. The MTL is generally categorized into two: joint training and multi-step training methods. DSS is one type of joint training method. In previous MTL works, the models share parts of layers. For the DSS, the two tasks share all weights of two tasks. Moreover, the objective of DSS is to improve the main task~(predicting task) and distill knowledge from auxiliary task~(explaining) instead of both tasks. 


\noindent\textbf{Information Bottleneck~(IB)} IB~\cite{tishby2015deep,slonim2002information} provides a powerful statistical tool to learn
representation to preserve complex intrinsic correlation
structures over high dimensional data. As a general measure of the
dependence between two random variables, MI is also widely used in deep learning to effectively represent feature dependencies~\cite{cover1999elements,covert2023learning,liu2009feature}. Estimating MI is known to be challenging, and recent progress has been made towards learning-based variational approaches~\cite{tian2019crd,covert2023learning,bachman2019learning,tschannen2019mutual,belghazi2018mutual,diao2023forward}. Another challenge associated with the IB principle is the optimization process, which involves a trade-off between achieving concise representation and maintaining strong predictive capabilities~\cite{alemi2016deep,wang2019deep}. 
%Another challenge of IB is that the optimization process is a trade-off between a concise representation and a good predictive power. 
%It leads to a problem of obtaining both high compression and accurate prediction~\cite{alemi2016deep,wang2019deep}. 
Consequently, optimizing IB becomes a complex task that heavily depends on the problem formulation and the provision of an effective optimization solution. Recent studies have applied IB to solve complex machine learning problems both in computer vision~\cite{tian2021farewell,du2020learning,wan2021multi} and NLP~\cite{chen2020learning,zhang2022improving,paranjape2020information}. In this paper, we formulate our CoT distillation problem with MTL training pipeline using IB method, and provide a learning-based solution to optimize IB for our CoT distillation, as detailed in Section~\ref{sec:meth}.
% Objective of DSS is to transfer knowledge of CoT generated large models to smaller models and improve these performance. Information theory provides a natural lens for quantifying the statistical relationship between these variables~\cite{cover1999elements,tishby2015deep}, and so is a common framework for deriving distillation losses in~\cite{zhang2022contrastive,miles2022itrd,passalis2020heterogeneous,aguilar2020knowledge}. The crucial issues are how to design and where apply to? In our proposed method, we develop a loss based on MI and apply it on last layers of two tasks because they are generally considered as task-oriented features. 

% In recent years, introducing information theory to model training losses has offered to new insights into deep learning~\cite{tishby2015deep,gabrie2018entropy}. 

% In the context of representation distillation, most losses can be modelled as maximising some lower bound on the MI between the student and the teacher models~\cite{tian2019contrastive,aguilar2020knowledge,chen2016infogan,chen2021wasserstein}.  Mutual information has been widely used for deep learning in a lot of tasks such as GAN~\cite{chen2016infogan}. However, estimating MI is challenging as we typically have access to samples but not the underlying distributions.  Most of existing methods focus on maximizing the MI between a learned representation and an aspect of the data with variational methods~\cite{hjelm2018learning,tian2021farewell,poole2019variational}. Compared with them, in this paper, we focus on maximizing MI between two learned representations of predicting task or explaining task.

% The most relevant idea to ours is the recent study~\cite{covert2023learning}, which inspired us for this work. However, there are three distinct differences: 1): In~\cite{covert2023learning}, the policy selection aims at reinforcement learning~(RL) but ours is self-learning with MTL framework; 2:) In~\cite{covert2023learning}, the task is classification of computer vision~(CV) and ours is LLM task and cam work on CV task as well. Obviously, our work is more general; and 3): In~\cite{covert2023learning}, the selection method is a binary mask $\{0,1\}$, and ours is continuous variable mask, which We can call it reweighing.
% However, the motivation behind \cite{chin2023prompting4debugging} is not from machine unlearning.
% Moreover, there exists another significant methodological difference.  
% Our proposed adversarial prompt generation method, termed {\ours}, 
% leverages the concept of the \textit{diffusion classifier} (utilizing the unlearned DM as a classifier). It provides computational efficiency without sacrificing effectiveness, setting it apart from the hard prompt optimization method \cite{wen2023hard} used in \cite{chin2023prompting4debugging}.
% Our research shows that adversarial prompts can be efficiently designed using the diffusion classifier and effectively used to evaluate the robustness of unlearned DMs. We refer readers to \textbf{Fig.\,\ref{fig: overview}} for a visual representation of the conceptual distinctions between our approach and existing works, as well as a demonstration of the attack performance of {\ours} against the Erased Stable Diffusion (ESD) model \cite{gandikota2023erasing}, which is one of the strongest unlearned DMs evaluated in our study.

==> intro.tex <==
\section{Introduction}
\label{sec:intro}
% Recently, Chain-of-Thought (CoT) prompting methods have shown language models models~(LMs) have exhibited enhanced reasoning capabilities in tackling complex reasoning tasks, owing to the utilization of a method named
% “Chain-of-Thought (CoT) prompting”.

%The capabilities of larger language models~(LLMs) grow with regarding to their size leading to considerable demand for resources~\cite{chowdhery2023palm}. Consequently, deploying these models in real world application is challenging, and the development of of efficient LLMs has become one of hot topics~\cite{wan2023efficient,yang2023harnessing,ding2023efficiency}.  

\begin{figure*}[!ht]
\vskip 0.2in
\begin{center}
% \centerline{\includegraphics[clip,trim= {.15\columnwidth} 0 {.15\columnwidth} 0, width=0.9\columnwidth]{icml2024/figure/scheme.png}}
\centerline{\includegraphics[width=1.8\columnwidth]{icml2024/figure/MI_overview.pdf}}
\caption{Overview on our approach: distilling step by step from an IB perspective and measuring intrinsic relationship between the two tasks by MI. The DSS is a MTL framework pipeline consisting of 
%two tasks: 
predicting and explaining tasks. 
%In the predicting task, the input is \textsc{[predict]+text} and output is label, and in the explaining task, the input is \textsc{[explain]+text} and output is rationale generated by CoT. 
Besides prediction loss and explanation losses used in DSS, we design an auxiliary loss,named MI loss, which aims to maximize the mutual information between the two representation features. In turns, CoT reasoning capacity can be enhanced by task-oriented distillation.}
\label{fig:scheme}
\end{center}
\vskip -0.2in
\end{figure*}

The capabilities of larger language models (LLMs) tend to scale with their model size, leading to a substantial demand for memory and compute resources~\cite{chowdhery2023palm,wei2022emergent}. Distilling knowledge from large LLMs to smaller LLMs has been pivotal for efficient AI deployment~\cite{Hinton2015distilling,phuong2019towards}. Chain-of-Thought (CoT)~\cite{wei2022chain} model distillation represents a pivotal advance in the quest to imbue smaller language models with the sophisticated reasoning capabilities of their larger counterparts. By distilling complex thought processes into more compact models, this approach aims to democratize access to advanced natural language understanding and reasoning across a wider array of computational resources.    %This poses challenges in the practical deployment of LLMs for real-world applications. 
%To circumvent these deployment challenges, recent research efforts~\cite{wan2023efficient,yang2023harnessing, ding2023efficiency} have pivoted towards efficient LLMs.
%the development of efficient LLMs has emerged as a critical area of focus in recent research, as highlighted by works such as \cite{wan2023efficient,yang2023harnessing, ding2023efficiency}.
%One main stream is knowledge distillation (KD), which transfers knowledge from larger, more competent teacher models into smaller student models affordable for practical applications~\cite{Hinton2015distilling,phuong2019towards}.
%Chain-of-thought (CoT), which prompts to breaks down complex tasks into smaller, more manageable steps, enhances LLM's problem solving ability 
%prompting has been proposed to improve LLMs' ability, 
%especially on the challenging arithmetic, commonsense, and symbolic reasoning tasks~\cite{wei2022chain}.
%, represents a significant advancement in enhancing the cognitive abilities of LLMs. 
%This approach involves a prompting mechanism that breaks down complex tasks into smaller, more manageable steps, thereby enhancing the effectiveness of the problem-solving process. 
However, it has been observed the CoT prompting methods on a model with less than 10 billion parameters may not only fail to enhance model performance but also potentially impair it~\cite{wei2022chain}. 
This challenge has spurred the exploration of training smaller language models that possess enhanced reasoning capabilities through CoT%, marking an exciting development in the field of efficient LLMs training
~\cite{ma2023sci,magister2023teaching,li2023symbolic}.

%Since its emerging~\cite{Hinton2015distilling}, Knowledge Distillation (KD) has been widely applied to a wide range of applications~\cite{phuong2019towards}.
%KD has become a powerful tool to transfer knowledge either in various ML tasks such as efficient AI for training smaller models~\cite{jiao2020tinybert}, MTL for enhancing main task training~\cite{yang2022cross}, and omin-supervision learning with data distillation~\cite{radosavovic2018data}.le
%Leveraging KD and CoT, a 
A recent research effort \textit{Distilling Step-by-Step}~(DSS)~\cite{hsieh2023distilling} proposes to efficiently train smaller student models %with shared weights 
guided by the rationales generated by a significantly larger teacher model, leveraging both CoT and KD. Instead of training both teacher and student models, it prompts the large teacher model to generate CoT rationales, and applies multi-task learning (MTL) framework to train a smaller models for both label and rationale prediction.  %generated from the teacher model are collected through employing CoT prompting. 
%In the online distillation stage, it applies multi-task learning~(MLT) to train a smaller student model to predict both labels and rationales.%, as shown in Figure~\ref{fig:scheme}. %Intuitively, rationales provide richer, more detailed information about why an input is mapped to a specific output label, allowing the small student model to forecast labels more accurately.
%Building on CoT reasoning, Hsieh et al.~\cite{hsieh2023distilling} have recently developed a novel two-step training pipeline, namely \textit{Distilling Step-by-Step}~(DSS). 
%This pipeline is designed to train smaller LMs more effectively or on less data. 
%In the first step of this process, a larger model, acting as a teacher, employs CoT prompting to generate both answers and rationales. 
%The second step involves applying multi-task learning~(MLT), aiming to minimize both label loss and rationale loss. 
%Essentially, DSS is an MLT task that enables the transfer of reasoning capabilities from LLMs to smaller LMs during the rationale prediction task. 
In this process, CoT knowledge is transferred through rationales generated by LLMs to smaller models via MTL.  
The smaller model enhances its reasoning capabilities by learning to predict rationales, which in turn improves its ability to predict labels accurately.
%as it demands fewer resources during training and leads to smaller models with enhanced reasoning ability. 
Different from conventional knowledge distillation~\cite{Hinton2015distilling}, larger teacher models perform inference only once to generate rationales, without any model updating in distillation. Only smaller student models are trained and optimized, leading to a smaller distillation cost. DSS thus offers significant benefits in terms of both efficiency and effectiveness.
%Obviously, this greatly reduces the demands for resources. 
% Through the transfer of CoT reasoning, smaller models can reach performance levels on reasoning tasks that were previously unattainable due to their inherent limitations. 
% This approach is particularly useful in scenarios with limited computational resources or where deploying large models is impractical due to processing or storage constraints.~\cite{brown2020language,zhao2023survey}. %Besides efficiency, the DSS framework enables a significant enhancement to the smaller models by imbuing them with the sophisticated reasoning capabilities typically associated with LLMs. 
% %It is worth noting that larger teacher models is only run forward part during the first step to generate rationales, while only the smaller models are run during training step.


% %Figure~\ref{fig:scheme} illustrates the DSS training process, in which the input text is combined with task prefixes \textsc{[predict]} and \textsc{[explain]}. These tokens signify two distinct tasks: label \textit{predicting} task and CoT rationale \textit{explaining} task, from the same input text. \hanxian{duplicated with the figure caption}
% While DSS aims to promote knowledge distillation for complex tasks, low-quality and noisy CoT rationales, and the intricacies in training models under the MTL framework could impact the effectiveness and reliability of the DSS process~\cite{wang-etal-2023-scott}. LLMs are prone to producing hallucinations and inconsistent rationales, which could potentially mislead the student model toward incorrect answers and cause conflicts in MTL that destruct student model learning~\cite{wang-etal-2023-scott,mueller2022text}.  

%Compared with general knowledge distillation, DSS adopts MTL framework to transfer the knowledge through the shared weights instead of two models. Consequently, we can consider the DSS as one type of self-distillation. However, previous self-distillation works train one larger model and improve some shallow sub-networks with task-orient the knowledge~\cite{zhang2019your, xu2019data,zhang2020task}. 

Research works of both MTL and KD have shown that introducing auxiliary losses improves performance of either main task of MTL or student models of distillation. However, DSS fails to bridge the predicting and explaining tasks. DSS aims to promote knowledge distillation for complex tasks, low-quality and noisy CoT rationales, and the intricacies in training models under the MTL framework could impact the effectiveness and reliability of the DSS process~\cite{wang-etal-2023-scott}. Furthermore, LLMs are prone to producing hallucinations and inconsistent rationales, which %could 
potentially mislead the student model toward incorrect answers and cause conflicts in MTL that destruct student model learning~\cite{mueller2022text}.

%To this end, 
To tackle the issues, we investigate the DSS from an information-theoretic viewpoint and develop a new auxiliary loss that aims to maximize the mutual information of the two tasks. %shared between the auxiliary task CoT rationale generation and the main task within an MTL framework. 
Our focus %is on 
lies in how the label-predicting task can generate representations that maximally align with those produced by the explaining task, thereby enhancing %the 
knowledge transfer from CoT. We conceptualize this relationship as task-oriented self-distillation, specifically designed to maximize mutual information (MI). MI plays a pivotal role in the quality of representations learned by these tasks. Despite the challenges in directly estimating MI, we draw inspiration from the methodology outlined in~\cite{covert2023learning} and propose a novel variational method to effectively maximize MI in the DSS context. 

We conduct comprehensive experiments with two smaller types of T5 models~\cite{2020t5}, T5-base~(220M) and T5-small~(60M), on four popular datasets. These datasets are e-SNLI~\cite{NIPS2018_8163}, ANLI~\cite{nie2019adversarial}, CQA~\cite{talmor-etal-2019-commonsenseqa} and SVAMP~\cite{patel-etal-2021-nlp}. Meanwhile, we provide deep and detailed analysis on Section~\ref{sec:discussion}. We believe that these results will be a guide for using DSS framework in the future.  

% The emergence of large language models (LLMs) has significantly revolutionized the NLP landscape, as highlighted by \citeauthor{brown2020language} and \citeauthor{zhao2023survey}. One of the key trends in this field is leveraging the capabilities of LLMs to unlock new applications, particularly in transferring the reasoning capacity of these models to smaller ones. This transfer is facilitated by the Distilling Step-by-Step (DSS) process, which utilizes a Multi-Task Learning (MTL) pipeline.  

%\citeauthor{wei2022chain} introduced Chain-of-thought as a powerful technique that enhances AI models' cognitive abilities by breaking down complex tasks into smaller steps. They point out that these prompting methods that are less than 10 billion parameters not only fail to enhance performance but can potentially impair it. As a result, training smaller LLM models that have reasoning capabilities via COT has evolved into intriguing research fields within the realm of efficient LLMs~\cite{ma2023sci,magister2023teaching,zhu2023survey,ding2023efficiency}. Compared with others, the most prominent benefits of DSS are efficient and effective, meaning less demand for resource during training and achieving smaller models with better accuracy.

%Introduced in~\cite{wei2022chain}, Chain-of-thought reasoning is

%Recently, Hsieh~\etal~\cite{hsieh2023distilling} has developed a simple two-step training pipeline, \textit{referring to as Distilling step-by-step~(DSS)}, to training smaller language models models~(LMs) on less data. The first step is data generation step, in which considering a larger model, as a teacher, Chain-of-Thought~(CoT) prompting is utilized to generate both answers and rationales. The second step is training step, in which multi-task learning~(MLT) is applied to minimize both label loss and rationale loss. DSS is de facto MLT task but can transfer the reasoning capabilities of LLMs into smaller model during training rationales predict task.


%Introduced in~\cite{wei2022chain}, Chain-of-thought reasoning is a powerful technique that enhances AI models' cognitive abilities by breaking down complex tasks into smaller steps. At the same time, Wei~\etal point out that these prompting methods that are less than 10 billion parameters not only fail to enhance performance but can potentially impair it. As a result, training smaller LLM models which have reasoning capabilities via COT has evolved into intriguing research fields within the realm of efficient LLMs~\cite{ma2023sci,magister2023teaching,zhu2023survey,ding2023efficiency}. Compared with others, the most prominent benefits of DSS are efficient and effective, meaning less demand for resource during training and achieving smaller models with better accuracy.
% Recent work have found that these CoT prompting methods are effective only for models with at least 10 billion of parameters~\cite{wei2022chain,Liu2023FederatedPA}. Leveraging MLT, the goal of DSS is to transfer 

%Since emergence of the LLMs the NLP landscape has been revolutionized~\cite{brown2020language,zhao2023survey}. Utilizing their new capacities to unlock new applications is a trend. Through MTL pipeline, DSS transfers reasoning capacity of COT generated by LLMs to small models.    

%Although success transferring capacities of COT of larger models, two things sounds be overlooked: noise label and how impacts of MLT because of the special relationship of the two tasks. As shown in Fig.~\ref{fig:scheme}, the training of SDD can be decomposed into two tasks, one refers to as predicting task, in in which the input is [PREDICT] + text and output is label and one refers to as explaining task, which the input is [EXPLAIN]+ text and the output is rationale. In the inference phase, only predicting task is evaluated. It is obvious that the explaining task is an auxiliary task in DSS. 
 
% Both MLT and noise label training are well-studied problems, and we also believe that some methods of MLT and noise label. However, this paper aims to analyze DSS which is a new scenario because of emerging of LLMs and focus on deeply understanding the method with perceptive of information theory. In term of it, we propose a new loss to improve the training pipeline.

% In terms of \cite{covert2023learning}, 





%Exploiting useful information contained in training tasks and formulating them into training paradigm are important in MTL. On the other hand, COT and the main task are not sufficient and necessary relationship. In this paper, we investigate properties of two tasks from an information-theoretic perspective. For better transferring knowledge from COT, the predicting task needs to generate representations that share maximum information with the representations generated by explaining task. Based on this intuition, we formulate the relationship between two task as dynamic feature selection through self-learning for maximizing mutual information~(MI), which plays an important role in the quality of the representations they learn.However, it is hard to directly estimate MI. In this paper, Inspired by learning method to maximize MI in~\cite{covert2023learning}, we propose a new variation method to maximize MI method. 
% Mutual information is a fundamental quantity that measures the relationship between random variables but it is notoriously difficult to measure. An exact estimate is only
%tractable for discrete variables or a small set of problems




The main contributions are summarized as below:
\begin{enumerate}
\item  We offer a critical reevaluation of the DSS framework, identifying and addressing its limitations by harnessing an information-theoretic viewpoint that underscores the synergy between label prediction and rationale explanation. 
\item Building on the theoretical foundation, we introduce an innovative auxiliary loss function designed to seamlessly integrate these two tasks. This methodological enhancement not only strengthens the connection between predicting and explaining within the DSS framework but also represents a significant leap forward in our ability to distill complex reasoning into more compact models. %We revisit the DSS training pipeline and formulate the two tasks, predicting and explaining tasks, from an information-theoretic perspective. Based on it, we improve DSS with an auxiliary loss that effectively bridge two tasks. % revisit is not a contribution 
\item  Our methodology demonstrably outperforms existing benchmarks across multiple datasets, evidencing the efficacy of our approach in enhancing the reasoning capabilities of distilled models. % Based on the proposed loss, our method substantially surpasses existing state-of-the-art approaches with significant improvement of most of the cases in four datasets. 
\item We systematically review predicted task and explainable tasks relationships under MTL training task with theoretical analysis results. To the best of our knowledge, it is the first work to quantitative analyze the models with CoT distillation. \hanxian{The last sentence is over-claimed?}
\end{enumerate}

% $$\underset{x \to \infty}{\lim}$$
% $\sum\limits_{j=0}^{3} {2 \above j}$ 

==> new_prelim.tex <==


% \subsection{Preliminaries}

In this section, we lay the foundation for our approach to mutual information-based distillation in a multi-task learning framework using the T5 model. We consider two primary tasks: label prediction and rationale generation, both derived from the same input. Our target smaller model, T5 and its variants, could be considered as a function mapping an input sequence of tokens to an output sequence of tokens.

Since mutual information is nonlinear and can effectively represent the dependencies of features, it is one of widely used measurements in feature selection

We denote $X$ as the input to the model. We define two random variables, $Y_1$ and $Y_2$, representing the outcomes of the label prediction and rationale generation tasks, respectively. The model estimates probability distributions for these tasks, $P_{\text{label}}(Y_1|X)$ for label prediction and $P_{\text{rationale}}(Y_2|X)$ for rationale generation. To adapt the input for MTL, we prepend task-specific prefixes \textsc{predict} and \textsc{explain} to $X$, resulting in modified inputs $X'_{\text{label}}$ and $X'_{\text{rationale}}$. Consequently, the probability distributions are denoted as $P_{\text{label}}(Y_1|X'_{\text{label}})$ and $P_{\text{rationale}}(Y_2|X'_{\text{rationale}})$ for label prediction and rationale generation tasks, respectively.


\subsection{Mutual-Information Based Distillation}
Our distillation process aims to train a smaller model to mimic the behavior of the LLM in performing these two tasks. The key metric guiding this process is the cross-entropy between the probability distributions of the label prediction and rationale generation tasks.

It is rare difficult to directly estimate mutual information in high dimension, especially when involving latent variable optimization

We propose the MI-based distillation approach aims to align the model's understanding and representation of the input $X$
X in such a way that it optimally informs both the label prediction and rationale generation tasks. 
The cross-entropy between these distributions is given by:
\begin{equation}
H(P_{\text{label}}, P_{\text{rationale}}) = -\sum_{y_1} P_{\text{label}}(y_1|X) \log P_{\text{rationale}}(y_1|X)
\end{equation}

This measure quantifies the expected number of additional bits required to identify an outcome of $Y_1$ using the probability distribution of $Y_2$, given the input $X$. Minimizing this cross-entropy is equivalent to maximizing the mutual information between the label prediction and rationale generation tasks, which can be conceptually represented as:
\begin{equation}
\max I(Y_1; Y_2) \approx \min H(P_{\text{label}}, P_{\text{rationale}})
\end{equation}

The distillation process involves adjusting the parameters of the smaller model to minimize the cross-entropy between the two probability distributions, thereby maximizing the mutual information between the label prediction and rationale generation tasks. %This approach ensures that the distilled model efficiently captures and leverages the shared information between these tasks. Next, we explain 

\subsection{A Variational Perspective on MI}

 In this section, we provide a variational perspective, specifically focusing on Conditional Mutual Information (CMI), to further refine our understanding of how information is shared and optimized in our multi-task learning framework using the T5 model. The CMI, denoted as $I(\mathbf{x_{i}}; \mathbf{y} | x_{s})$, is a pivotal concept in dynamically selecting features or tokens that are most informative for tasks, in our work, the label prediction and rationale generation tasks.

In this framework, $x_{s}$ represents the subset of features already selected, $\mathbf{x_{i}}$ represents a candidate feature for selection, and $\mathbf{y}$ represents the output variable, which could be either the label prediction ($Y_1$) or the rationale generation ($Y_2$), depending on the task. The CMI is defined as the KL divergence between the joint and factorized distributions of these variables:
\begin{equation}
I(\mathbf{x_{i}}; \mathbf{y} | x_{s}) = D_{KL}(p(\mathbf{x_{i}}, \mathbf{y} | x_{s}) || p(\mathbf{x}_{i} | x_{s}) p(\mathbf{y} | x_{s}) )
\end{equation}

The feature selection policy, $\phi(x_s)$, aims to minimize this CMI, effectively choosing features that maximize the information about the output variable $\mathbf{y}$. This approach aligns with our objective of distilling and transferring knowledge efficiently in the multi-task T5 framework, where the internal representation of input tokens play a crucial role in predicting both labels and generating rationales.

The prediction function $f$, in the context of T5, is defined as:
\begin{equation}
f(x_{s}) = p(\mathbf{y} | x_{s})
\end{equation}
representing the model's probability estimation of the output given the selected features.

Following the methodologies outlined in ~\cite{covert2023learning,poole2019variational}, we estimate the CMI by calculating the mean KL divergence relative to the model's prediction across different subsets of features:
\begin{equation}
\label{eq:mean}
M_{i}^{n} = \frac{1}{n} \sum_{j=1}^n D_{KL}(p(\mathbf{y} | x_{s}, x_{i}^j) || \frac{1}{n} \sum_{l=1}^n p(\mathbf{y} | x_{s}, x_{i}^l) )
\end{equation}
This estimation process allows us to approximate CMI practically and efficiently, facilitating the dynamic selection of features in our model. Ultimately, as proposed by \cite{covert2023learning}, the limit of this CMI estimator as $n \to \infty$ approaches the true CMI:
\begin{equation}
\lim _{n \to \infty} I_{i}^n = I(\mathbf{y}; \mathbf{x}_{i} | x_{s})
\end{equation}

This variational perspective on mutual information is crucial in our multi-task learning setting. It guides the selection method as an optimization problem, aiming to minimize the expected loss of the model's prediction. The expected loss for adding a new feature $\mathbf{x}{i}$ to the current set $x{s}$ is represented as:
\begin{equation}
\label{eq:expection}
\mathbb{E}_{\mathbf{y}, \mathbf{x}_{i} | x_{s}} = [l(f(x_{s} \cup \mathbf{x}_{i}), \mathbf{y})]
\end{equation}
In the context of MLT framework with T5, the expected loss (if defined in terms of cross-entropy) would guide the feature selection process to minimize the average discrepancy in predictions across different tasks. This formulation aligns with our overarching goal of enhancing the T5 model's efficiency in handling multiple tasks by optimally selecting the most informative features for label prediction and rationale generation.

In terms of the Blahut–Arimoto algorithm, we can obtain
\begin{proposition}
    When $\mathbf{y}$ is discrete, $l$ is cross-entropy loss.The $f$ is the explaining model, and Eq.~\ref{eq:expection} is minimized by predicting model or equal to $\arg max_{i}I(\mathbf{y}; \mathbf{x}_{i} | x_{s})$.
\end{proposition}
In terms of it, the self-learning process is equivalent to minimizing the one-step-ahead loss.
    




==> old_prelim.tex <==
%Let $\mathbf{x} = (\mathbf{x}_{1}, ...,~\mathbf{x}_{d})$ denotes a vector of input features with dimension $d$, and $\mathbf{y}$ a response variable for a supervised learning task. We notate $s \subseteq [d] \equiv \{1,...d\}$ to denote a subset of indices and $\mathbf{x}_{s} = \{ \mathbf{x}_{i}: i \in s \}$ a subset of features. Bold symbols $\mathbf{x},\mathbf{y}$ represent random variables. The symbols $x,y$ are possible values, and  $p(\mathbf{x},\mathbf{y})$ denotes the \textcolor{red}{joint distribution of(?)} data. 

%Our goal is to design a method to control which features are selected or weighted given the  currently available information. The selection method can be viewed as function $\phi(x_s) \in [d]$, meaning that it selects a subset of features as its input. 

Given a network $f$ and s subset of dataset $x_{s}$, the predicted result can be written as 
\begin{equation}
\label{eq:cost}
% \hat{y} = f(\{x_{i_{t}}\}^{k}_{t=1})
\hat{y} = f(x_{s})
\end{equation}

Given a loss function $l(\hat{y}, y)$ that measures prediction $\hat{y}$ and labels $y$. The cost function is defined as a a policy-predictor pair $(\phi,f)$ as follows:
 \begin{equation}
\label{eq:cost}
% \mathbf{\rho_{k}(\phi,f)} = \mathbb{E}_{p(x,y)}[l(f(\{x_{i_{t}}\}^{k}_{t=1}), \mathbf{y})]
\mathbf{C(\phi,f)} = \mathbb{E}_{p(x,y)}[l(f(x_{s}), \mathbf{y})]
\end{equation}
The goal is to minimize cost function, or to maximize our final predictive accuracy. 

\subsection{A Variational Perspective on MI}
\label{sec:Variation}
The CMI, denoted as $I(\mathbf{x_{i}}; \mathbf{y} | x_{s})$, is defined as the KL divergence between the joint and factorized distributions \textcolor{red}{ of what? }:
\begin{equation}
    I(\mathbf{x_{i}}; \mathbf{y} | x_{s}) = D_{KL}(p(\mathbf{x_{i}}; \mathbf{y} | x_{s}) || p(\mathbf{x}_{i} | x_{s}) p(\mathbf{y} | x_{s}) )
\end{equation}
where the policy as $\phi(x_s) \equiv \arg\min_{i} I(\mathbf{x_{i}}; \mathbf{y} | x_{s}) $, so that features are sequentially selected as to maximize the information about the response variables. The function $f$ is considered as with 
\begin{equation}
    f(x_{s}) = p(\mathbf{y} | x_{s})
\end{equation}
According to ~\cite{covert2023learning,poole2019variational}, We calculate the mean prediction and the mean of KL divergence relative to this prediction, which yields to the CMI estimator as following:
\begin{equation}
\label{eq:mean}
    M_{i}^{n} = \frac{1}{n} \sum_{j=1}^n D_{KL}(p(\mathbf{y} | x_{s}, x_{i}^j) || \frac{1}{n} \sum_{l=1}^n p(\mathbf{y} | x_{s}, x_{i}^l) )
\end{equation}
In terms of \cite{covert2023learning}, the solution of limiting result of Equation~\ref{eq:mean}
\begin{equation}
    \lim _{n \to \infty} I_{i}^n = I(\mathbf{y}; \mathbf{x}_{i} | x_{s})
\end{equation}
% % According to IB priciple~\cite{tishby2015deep}, Given data 
% The goal of dynamic feature selection features with minimal budget that achieve
% The CMI, denoted as $I$

For our propose, the selection method can be viewed as an optimization problem, the expected loss of one step is written as:
% \begin{euqation}
%      \mathbb{E}_{\mathbf{y}, \mathbf{x}_{i} | x_{s}}[l(f(x_{s}), \mathbf{y})
% \end{euqation}
\begin{equation}
    \mathbb{E}_{\mathbf{y}, \mathbf{x}_{i} | x_{s}} = [l(f(x_{s} \cup \mathbf{x}_{i}), \mathbf{y})]
\end{equation}

